Computational Complexity of the Bondage Problem

For a graph $G$, the domination number $\gamma(G)$ is the minimum size of a vertex set that dominates all vertices of $G$. The bondage number $b(G)$ is the minimum number of edges whose deletion increases the domination number. The $d$-Bondage problem asks, given a graph $G$ and an integer $d$, whether $b(G)\leq d$. The precise computational complexity of Bondage has remained open. Most recently, Bakal and Borse have shown that even $1$-Bondage is both $\mathrm{NP}$-hard and $\mathrm{coNP}$-hard. We show that, for every fixed integer $d\geq 1$, $d$-Bondage is $\Theta_2^{\mathrm{P}}$-complete even on chordal graphs, and that the general Bondage problem is $\Sigma_2^{\mathrm{P}}$-complete. We then study the parameterized complexity of Bondage. On the positive side, we give fixed-parameter algorithms parameterized by the treewidth of the input graph alone, by the cluster vertex deletion number plus $d$, and by the neighborhood diversity plus $d$. In contrast, parameterization by the domination number does not lead to tractability: Bondage is $\mathrm{para\text{-}NP}$-hard parameterized by $\gamma(G)$, and remains $\mathrm{W}[1]$-hard parameterized by $\gamma(G)$ even when $d=1$. More precisely, the problem is polynomial-time solvable when $\gamma(G)=1$, but becomes $\mathrm{NP}$-hard already on split graphs with $\gamma(G)=2$. These results determine the classical complexity of Bondage within the polynomial hierarchy and give a broad picture of its parameterized complexity under natural graph parameters.

==> conc.tex <==
\section{Concluding Remarks}
We establish $\ThetaTwoP$-completeness for every fixed $d$ and
$\SigmaTwoP$-completeness when $d$ is unrestricted, leaving the
complexity of intermediate regimes such as $d=O(\log n)$ open.
Interestingly, the classification obtained here does not exhibit a
$\DeltaTwoP$-complete regime: fixed $d$ yields $\ThetaTwoP$-completeness,
whereas unrestricted $d$ yields $\SigmaTwoP$-completeness.
It is therefore natural to ask whether some intermediate restriction on the growth of $d$
leads to $\DeltaTwoP$-completeness or to a class characterized by limited nondeterminism.

On the parameterized side, our results leave several gaps in the
complexity landscape of Figure~\ref{fig:overview}.
In particular, it is not known whether \bondage is fixed-parameter
tractable parameterized by $\operatorname{cw}(G)+d$.
For treewidth $k$, our algorithm has a doubly exponential dependence
on $k$.

Doubly exponential dependence on treewidth is known to be unavoidable
under ETH even for natural problems at the second level of the polynomial
hierarchy; in particular, Lampis and Mitsou established such a lower bound
for $\exists\forall$-SAT~\cite{DBLP:conf/iwpec/LampisM17}.
Related doubly exponential lower bounds are also known for
3-Choosability~\cite{DBLP:conf/icalp/MarxM16}.
This makes it natural to ask whether the doubly exponential dependence
for \bondage is inherent as well. 
Our present $\SigmaTwoP$-hardness reduction, however, is not designed
to preserve bounded treewidth, and does not seem to yield such a lower
bound directly. Indeed, the constructed graph already contains cliques
of size linear in the number of existential variables. 
Thus, obtaining a $2^{2^{o(\mathrm{tw}(G))}}n^{O(1)}$ lower bound under ETH, or
alternatively a substantially faster treewidth-based algorithm, remains
an interesting open direction.

==> hardness.tex <==
%\section{Hardness results}
\section{Classification within the second level of the polynomial hierarchy}\label{sec:ph}
In this section, we determine the complexity of \bondage within the
second level of the polynomial hierarchy.  We first consider the case
where the deletion bound $d$ is fixed, and then turn to the general
case where $d$ is part of the input.

\subsection{Completeness for \ThetaTwoP}
%In \cite{DBLP:conf/iwoca/BakalB26}, Bakal and Borse resolved in the affirmative a conjecture of Hu and Xu~\cite{DBLP:journals/jc/HuX12} stating that \bondage is not in \NP, under the standard complexity assumption that $\NP \neq \coNP$.
%They proved that \onebondage is both \NP-hard and \coNP-hard.
%In this subsection, we show that \onebondage is complete for the complexity class \ThetaTwoP, which lies at the second level of the polynomial hierarchy.
%This strengthens the result of Bakal and Borse and completely determines the computational complexity of \onebondage.
We begin with the case where the deletion bound $d$ is fixed. 
\begin{definition}[\cite{DBLP:journals/siamcomp/Wagner90}]
  The computational complexity class \ThetaTwoP, also denoted by $\P^{\NP[\mathcal{O}(\log{n})]}$, is the class of languages decidable by a deterministic polynomial-time Turing machine that makes $\mathcal{O}(\log{n})$ queries to an {\NP} oracle.
\end{definition}

\begin{theorem}\label{thm:theta2p-membership}
  For every fixed integer $d \geq 1$, \dbondage belongs to \ThetaTwoP.
\end{theorem}
\begin{proof}
    For a fixed integer $d \geq 1$, given a graph $G$ and an integer $\ell$, consider the problem of deciding whether $\gamma(G-F) \leq \ell$ for every $F \subseteq E(G)$ with $|F| \leq d$.
    This problem is in \NP: since $d$ is fixed, there are only polynomially many such sets $F$, and a certificate consists of a dominating set of size at most $\ell$ for each $G-F$.
    We compute $\gamma(G)$ by binary search using $\mathcal{O}(\log{|V(G)|})$ \NP-oracle queries and then make one additional query to the above problem with $\ell = \gamma(G)$.
    Since deleting edges cannot decrease the domination number, $b(G) \leq d$ if and only if this final oracle query returns no.
    Hence \dbondage belongs to \ThetaTwoP.
\end{proof}

\begin{remark}
    The proof of \Cref{thm:theta2p-membership} relies crucially on $d$ being fixed.
    Indeed, if $d$ is part of the input, there may be exponentially many subsets $F \subseteq E(G)$ with $|F| \leq d$.
    Therefore, this argument does not extend to the general \bondage problem in which $d$ is part of the input.
\end{remark}

We next turn to the hardness proof. For this purpose, we use the following notions.
For a graph $G$, let $\tau\emph{-anticore}(G)$ denote the set of vertices contained in no minimum vertex cover of $G$.
We reduce from $\tau\textsc{-Anticore}$, which asks whether $|\tau\text{-anticore}(G)| \geq 1$.
A graph $G$ is $\tau\emph{-vertex-critical}$ (called $\beta\emph{-vertex-critical}$ in \cite{DBLP:journals/algorithmica/BurjonsFHKW24}) if $\tau(G - v) < \tau(G)$ for every vertex $v \in V(G)$.
Burjons, Frei, Hemaspaandra, Komm, and Wehner proved that recognizing $\tau\text{-vertex-critical}$ graphs is \ThetaTwoP-complete~\cite[Theorem 18]{DBLP:journals/algorithmica/BurjonsFHKW24}.
Observe that $\tau(G-v)<\tau(G)$ if and only if $v$ belongs to some minimum vertex cover of $G$.
Thus, $G$ is $\tau$-vertex-critical if and only if $\tau\text{-anticore}(G)=\emptyset$.
Since $\ThetaTwoP$ is closed under complementation, $\tau$-\textsc{Anticore} is $\ThetaTwoP$-complete.

Let $G$ be an instance of $\tau$\textsc{-Anticore}.
We construct a graph $H$ as follows (see \Cref{fig:theta2p:2}):
\begin{enumerate}
    \item For each $v \in V(G)$, add a clique $C_v$ of size $2d + 1$.
    \item For each $e = \{u, v\} \in E(G)$, add two vertices $x_e$ and $y_e$, each adjacent to every vertex in $C_u \cup C_v$.
    \item For each $v \in V(G)$, add a vertex $a_v$ adjacent to every vertex in $C_v$, and a clique $B_v$ of size $2d-1$ such that $a_v$ is adjacent to every vertex in $B_v$.
    \item Make $\bigcup_{v \in V(G)}{C_v}$ a clique.
\end{enumerate}
This completes the construction.
\begin{figure}
  \centering
  \includegraphics[page=2]{images/theta2p_fullpaper.pdf}
  \caption{An example of a graph $G$ and the corresponding graph $H$. Each dashed circle encloses a clique. Thick edges indicate complete connections between their endpoints, meaning that every vertex in a clique at one endpoint is adjacent to every vertex in the clique or the individual vertex at the other endpoint.}
  \label{fig:theta2p:2}
\end{figure}

We first show that $H$ is chordal.
Consider the following vertex ordering.
First, eliminate all vertices $x_e$ and $y_e$.
Then, for each $v \in V(G)$, eliminate all vertices in $B_v$, followed by $a_v$.
Finally, eliminate all vertices in $\bigcup_{v \in V(G)} C_v$.
It is easy to verify that this ordering is a perfect elimination ordering of $H$, and thus $H$ is chordal.

For each $v \in V(G)$, let $R_v = B_v \cup \{a_v\}$, and let $R = \bigcup_{v \in V(G)} R_v$.
The construction yields the following observation.
\begin{observation}\label{obs:theta2p}
    For any dominating set $D$ of $H$, there exists a vertex cover $S$ of $G$ satisfying the following properties:
    \begin{enumerate}
        \item $|S| \leq |D \setminus R|$,
        \item $D \cap C_v \neq \emptyset \implies v \in S \quad (v \in V(G))$.
    \end{enumerate}
\end{observation}
\begin{proof}
    Let $D$ be a dominating set of $H$.
    Since every vertex in $B_v$ has no neighbors outside $R_v$, we have $D \cap R_v \neq \emptyset$ for each $v \in V(G)$.
    Moreover, since $N[b] \subsetneq N[a_v]$ for every $b \in B_v$, we may replace any vertex in $B_v \cap D$ with $a_v$ without losing the domination property or increasing the size of $D$.
    Similarly, if $x_e$ or $y_e$ belongs to $D$ for some $e = \{u, v\} \in E(G)$, we may replace it with an arbitrary vertex in $C_u \cup C_v$.

    Let $D'$ be the resulting dominating set.
    Then, $D'$ consists of all vertices $a_v$ and some vertices in $\bigcup_{v \in V(G)} C_v$.
    Furthermore, these replacements preserve all vertices in $D \cap C_v$ for each $v \in V(G)$.

    Let $S = \{v \in V(G) \mid C_v \cap D' \neq \emptyset \}$.
    Since $D'$ dominates $x_e$ and $y_e$ for each $e = \{u, v\} \in E(G)$, we have $D' \cap (C_u \cup C_v) \neq \emptyset$.
    Hence, $S$ is a vertex cover of $G$.
    Both properties follow immediately from the construction.
\end{proof}


We next establish the following equality.
Let $n = |V(G)|$.
\begin{lemma}\label{lem:theta2p:1}
    $\gamma(H) = n + \tau(G)$.
\end{lemma}
\begin{proof}
    We first prove that $\gamma(H) \leq n + \tau(G)$.
    Let $S \subseteq V(G)$ be a minimum vertex cover of $G$ with $|S| = \tau(G)$.
    We construct a vertex set $D$ as follows:
    for each $v \in S$, add an arbitrary vertex $c_v \in C_v$;
    then, add $a_v$ for each $v \in V(G)$.
    Clearly, $|D| = n + \tau(G)$.
    We claim that $D$ is a dominating set of $H$.
    For each $v \in V(G)$, every vertex in $B_v \cup C_v$ is dominated by $a_v$.
    For each $e = \{u, v\} \in E(G)$, since $S$ is a vertex cover of $G$, at least one of $u$ and $v$ belongs to $S$.
    Thus, both $x_e$ and $y_e$ are dominated by a vertex in $D \cap (C_u \cup C_v)$.
    Therefore, $D$ is a dominating set of $H$, and hence $\gamma(H) \leq |D| = n + \tau(G)$.
    
    We next prove that $\gamma(H) \geq n + \tau(G)$.
    Let $D$ be a minimum dominating set of $H$.
    By \Cref{obs:theta2p}, there exists a vertex cover $S$ of $G$ with $|S| \leq |D \setminus R|$.
    Thus, we have $\tau(G) \leq |S| \leq |D \setminus R| \leq |D| - n = \gamma(H) - n$.
    This proves the lemma.
\end{proof}

\begin{lemma}\label{lem:theta2p:2}
    $\tau\text{-anticore}(G) \neq \emptyset$ if and only if $b(H) \leq d$.
\end{lemma}
\begin{proof}
    Suppose first that $\tau\text{-anticore}(G) \neq \emptyset$ and let $v \in \tau\text{-anticore}(G)$.
    Since $H[R_v]$ is a clique of size $2d$, it has a perfect matching $M$ with $|M| = d$.
    Let $D$ be a minimum dominating set of $H - M$.
    Clearly, $D$ is also a dominating set of $H$.

    Suppose that $D \cap C_v \neq \emptyset$.
    By \Cref{obs:theta2p}, there exists a vertex cover $S$ of $G$ such that $|S| \leq |D \setminus R|$ and $v \in S$.
    Since $v \in \tau\text{-anticore}(G)$, we have $|S| \geq \tau(G) + 1$.
    Moreover, since $D \cap R_u \neq \emptyset$ for every $u \in V(G)$, we have $|D \setminus R| \leq |D| - n$.
    Therefore, $\gamma(H-M) = |D| \geq n + |S| \geq n + \tau(G) + 1 = \gamma(H)$ + 1.

    Suppose otherwise that $D \cap C_v = \emptyset$.
    We claim that $|D \cap R_v| \geq 2$.
    Indeed, $H[R_v]-M$ is a clique with a perfect matching removed, and thus no single vertex in $R_v$ dominates all of $R_v$ in $H-M$.
    Since the only neighbors of vertices in $R_v$ outside $R_v$ belong to $C_v$, and $D \cap C_v = \emptyset$, we obtain $|D \cap R_v| \geq 2$.
    Since $D \cap R_u \neq \emptyset$ for every $u \in V(G)$, we have $|D \setminus R| \leq |D| - (n+1)$.
    By \Cref{obs:theta2p}, there exists a vertex cover $S$ of $G$ with $|S| \leq |D \setminus R|$.
    Hence, $\gamma(H-M) = |D| \geq n + |S| + 1  \geq n + \tau(G) + 1 = \gamma(H) + 1$.
    Therefore, in both cases, we have $\gamma(H-M) > \gamma(H)$, and hence $b(H) \leq |M| = d$.

    Conversely, suppose that $\tau\text{-anticore}(G) = \emptyset$.
    We show that $\gamma(H-F) = \gamma(H)$ for every $F \subseteq E(H)$ with $|F| \leq d$.
    For each $v \in V(G)$, since $|C_v| = 2d+1$ and $|F| \leq d$, there exists a vertex $c_v \in C_v$ incident with no edge of $F$.
    
    Suppose first that, for every $v \in V(G)$, there is a vertex $q_v \in R_v$ incident with no edge of $F$.
    Let $S$ be an arbitrary minimum vertex cover of $G$ and let $D' = \{q_v \mid v \in V(G)\} \cup \{c_v \mid v \in S\}$.
    Since each $q_v$ dominates all vertices in $R_v$, and the vertices $c_v$ with $v \in S$ dominate all vertices in $\bigcup_{v \in V(G)} C_v$ and all vertices $x_e$ and $y_e$, the set $D'$ is a dominating set of $H-F$ with $|D'| = n + \tau(G)$.

    Suppose otherwise that there exists a vertex $v \in V(G)$ such that every vertex in $R_v$ is incident with an edge of $F$.
    Since $|R_v| = 2d$ and $|F| \leq d$, this is possible only when $|F| = d$ and $F$ is a perfect matching of $H[R_v]$.
    Let $p_v \in B_v$ be the vertex matched with $a_v$ in $F$.
    Since $\tau\text{-anticore}(G) = \emptyset$, there exists a minimum vertex cover $S_v$ of $G$ containing $v$.
    Let $D' = \{a_u \mid u\neq v\} \cup \{p_v\} \cup \{c_u \mid u \in S_v\}$.
    Since $p_v$ dominates all vertices in $B_v$ and $c_v$ dominates $a_v$, every vertex in $R_v$ is dominated by $D'$.
    Thus, $D'$ is a dominating set of $H-F$ with $|D'| = n + \tau(G)$.
    
    In both cases, we have $\gamma(H - F) \leq n + \tau(G) = \gamma(H)$.
    Since deleting edges cannot decrease the domination number, we obtain $\gamma(H-F) = \gamma(H)$.
    Hence, $b(H) > d$.
\end{proof}

From \Cref{lem:theta2p:1,lem:theta2p:2}, the following holds.

\begin{theorem}\label{thm:theta2p-hardness}
    For every fixed integer $d \geq 1$, \dbondage is \ThetaTwoP-hard even when restricted to chordal graphs.
\end{theorem}

Finally, from \Cref{thm:theta2p-membership,thm:theta2p-hardness}, the following holds.
\begin{theorem}\label{thm:theta2p-completeness}
    For every fixed integer $d \geq 1$, \dbondage is \ThetaTwoP-complete even when restricted to chordal graphs.
\end{theorem}

\subsection{Completeness for $\SigmaTwoP$}

\begin{theorem}
  \bondage is \SigmaTwoP-complete.
\end{theorem}
\begin{proof}
    Membership in \SigmaTwoP is immediate: nondeterministically guess an edge set $F$ with $|F| \leq d$ and compare $\gamma(G-F)$ and $\gamma(G)$ using an \NP-oracle.

    We now prove the \SigmaTwoP-hardness.
    We reduce from $\textsc{QSAT}_2$ restricted to 3-DNF formulas.
    $\textsc{QSAT}_2$ asks whether there exists an assignment to variables in $X$ such that $\Phi(X,Y)$ is true for every assignment to variables in $Y$. 
    Let $\Phi(X, Y) = T_1 \lor \cdots \lor T_\ell$, $X = \{x_1, \dots, x_n\}$, $Y = \{y_1, \dots, y_m\}$.
    It is known that $\textsc{QSAT}_2$ is \SigmaTwoP-complete even when restricted to 3-DNF formulas~\cite{DBLP:journals/tcs/Marx08}.
    We may assume that $n \geq 1$, and identify true and false with $1$ and $0$, respectively.

    \paragraph{Construction.}
    We now construct an instance $\langle{G, d}\rangle$ of \bondage from $\langle{X, Y, \Phi(X, Y)}\rangle$.
    Let $M = 2n + 1$.
    We first construct a graph $G$ as follows (see \Cref{fig:sigma2p}):
    \begin{enumerate}
        \item For each $1 \leq i \leq n$, add vertices $x_i, \bar{x}_i, a_i, d_i^1, \dots, d_i^M$, and make them a clique.
        \item For each $1 \leq i \leq n$, add two vertices $p_i$ and $q_i$, each adjacent to all vertices in $\{x_i, \bar{x}_i, a_i, d_i^1, \dots, d_i^M\}$.
        \item For each $1 \leq i \leq n$, add a vertex $h_i$ adjacent to both $x_i$ and $\bar{x}_i$.
        \item For each $1 \leq j \leq m$, add vertices $y_j, \bar{y}_j, e_j^1, \dots, e_j^M$, and make them a clique.
        \item For each $1 \leq j \leq m$, add two vertices $r_j$ and $s_j$, each adjacent to all vertices in $\{y_j, \bar{y}_j, e_j^1, \dots, e_j^M\}$.
        \item For each $1 \leq s \leq \ell$, add a vertex $c_s$ adjacent to every literal vertex corresponding to the complement of a literal appearing in $T_s$.
        \item For each $1 \leq i \leq n$, add edges between $a_i$ and all vertices in $\{h_1, \dots, h_n,$ $c_1, \dots,  c_\ell\}$.
    \end{enumerate}
    Finally, set $d = n$.
    This completes the construction.
    \begin{figure}[htbp]
        \centering
        \includegraphics[page=1]{images/sigma2p.pdf}
        \caption{An example of the graph $G$ corresponding to $\Phi = (x_1 \land \bar{x}_2 \land y_2) \lor (x_1 \land x_3 \land \bar{y}_2) \lor (\bar{x}_1 \land \bar{x}_2 \land y_1)$. The vertices $\{x_i, \bar{x}_i, a_i, d_i^1, \dots, d_i^M, p_i, q_i\}$ form a clique minus the edge $\{p_i, q_i\}$, and the vertices $\{y_j, \bar{y}_j, e_j^1, \dots, e_j^M, r_j, s_j\}$ form a clique minus the edge $\{r_j, s_j\}$.}
        \label{fig:sigma2p}
    \end{figure}

    The construction yields the following observation.
    \begin{observation}\label{obs:sigma2p-complete}
        We have $\gamma(G) = n + m$.
        Moreover, every minimum dominating set consists of exactly one vertex from each of the sets $\{x_i, \bar{x}_i, a_i, d_i^1, \dots, d_i^M\}$ for all $i$ and $\{y_j, \bar{y}_j, e_j^1, \dots, e_j^M\}$ for all $j$.
    \end{observation}
    \begin{proof}
        We first show that $\gamma(G) \geq n + m$.
        Let $D$ be a dominating set of $G$.
        For each $1 \leq i \leq n$, $D$ must contain at least one vertex from $\{x_i, \bar{x}_i, a_i, d_i^1, \dots, d_i^M, p_i, q_i\}$ since both $p_i$ and $q_i$ are adjacent only to vertices in the set.
        Similarly, for each $1 \leq j \leq m$, $D$ must contain at least one vertex from $\{y_j, \bar{y}_j, e_j^1, \dots, e_j^M, r_j, s_j\}$.
        Since these sets are pairwise disjoint, $|D| \geq n + m$.
        
        Conversely, the set $\{a_1, x_2, \dots, x_n, y_1, \dots, y_m\}$ is a dominating set of size $n + m$.
        Indeed, it is easy to check that all vertices in the sets $\{x_i, \bar{x}_i, a_i, d_i^1, \dots, d_i^M, p_i, q_i\}$ and $\{y_j, \bar{y}_j, e_j^1, \dots, e_j^M, r_j, s_j\}$ are dominated, and all vertices $h_1, \dots, h_n$ and $c_1, \dots, c_\ell$ are dominated by $a_1$.
        Therefore, $\gamma(G) \leq n + m$, and hence $\gamma(G) = n + m$.
        
        By the above, every minimum dominating set $D$ consists of exactly one vertex from each of the sets $\{x_i, \bar{x}_i, a_i, d_i^1, \dots, d_i^M, p_i, q_i\}$ for all $i$ and $\{y_j, \bar{y}_j, e_j^1, \dots, e_j^M, r_j, s_j\}$ for all $j$.
        The vertices $p_i$ and $q_i$ are adjacent only to $\{x_i, \bar{x}_i, a_i, d_i^1, \dots, d_i^M\}$ and not adjacent to each other.
        Hence, in order to dominate both $p_i$ and $q_i$, neither $p_i$ nor $q_i$ can belong to $D$; otherwise, the other vertex would not be dominated.
        The same argument applies to $r_j$ and $s_j$.
        This proves the observation.
    \end{proof}

    \paragraph{Completeness.}
    Suppose that $\langle{X, Y, \Phi(X, Y)}\rangle$ is a $\mathrm{yes}$-instance, and let $\varphi_X$ satisfy $\Phi(\varphi_X,\varphi_Y)=1$ for every $\varphi_Y$.
    We construct an edge set $F$ by choosing, for each $1 \leq i \leq n$, $\{a_i, \bar{x}_i\}$ if $\varphi_X(x_i) = 1$, otherwise $\{a_i, x_i\}$.
    Clearly, $|F| = n$.

    Suppose that $G-F$ has a dominating set $D$ of size $n + m$.
    Since $D$ is also a minimum dominating set of $G$, \Cref{obs:sigma2p-complete} implies that $D$ consists of exactly one vertex from each of the sets $\{x_i, \bar{x}_i, a_i, d_i^1, \dots, d_i^M\}$ for all $i$ and $\{y_j, \bar{y}_j, e_j^1, \dots, e_j^M\}$ for all $j$.
    Neither $a_i$ nor the other endpoint of the edge in $F$ incident to $a_i$ belongs to $D$: otherwise, the other endpoint is not dominated by $D$ in $G-F$.
    Moreover, in order to dominate $h_i$, none of the copy vertices $d_i^1, \dots, d_i^M$ can belong to $D$.
    Thus, for each $i$, $D$ contains exactly one of $x_i$ and $\bar{x}_i$, namely the literal vertex that evaluates to true under $\varphi_X$.

    We now define an assignment $\varphi_Y$ as $\varphi_Y(y_j) = 1$ if and only if $y_j \in D$.
    Since $D \cap \{c_1, \dots, c_\ell\} = \emptyset$, every term vertex $c_t$ is dominated by a literal vertex in $D$.
    Thus, there exists a literal vertex in $D$ that is adjacent to $c_t$, and this vertex represents a literal that evaluates to true under the assignment $\varphi_X$ and $\varphi_Y$.
    By construction of $G$, the term $T_t$ contains a complementary literal, which evaluates to false under the assignment $\varphi_X$ and $\varphi_Y$, contradicting $\Phi(\varphi_X, \varphi_Y) = 1$.
    Thus, we obtain $\gamma(G-F) > n + m = \gamma(G)$.

    \paragraph{Soundness.}
    Conversely, suppose that $\langle{X, Y, \Phi(X, Y)}\rangle$ is a $\mathrm{no}$-instance.
    We now show that for every $F \subseteq E(G)$ with $|F| \leq n$, $\gamma(G-F) = n + m = \gamma(G)$.
    We first observe that, since each set of copy vertices $\{d_i^1, \dots, d_i^M\}$ contains $M = 2n + 1$ vertices, there exists a vertex $d_i \in \{d_i^1, \dots, d_i^M\}$ incident to no edge in $F$.
    The same holds for $\{e_j^1, \dots, e_j^M\}$, and denote such vertex by $e_j \in \{e_j^1, \dots, e_j^M\}$.

    Suppose that there exists $a_{i_0}$ that is incident to no edge in $F$.
    Then, the set $\{a_{i_0}\} \cup \{d_i \mid 1 \leq i \leq n, i  \neq i_0\} \cup \{e_j \mid 1 \leq j \leq m\}$ is a dominating set of $G-F$ of size $n + m$.

    Otherwise, every $a_i$ is incident to at least one edge in $F$.
    Then, $|F| = n$ and exactly one edge $f_i \in F$ is incident to each $a_i$.
    Define an assignment $\varphi_X$ as $\varphi_X(x_i) = 1$ if and only if $f_i$ is not incident to $x_i$.
    Since $\langle{X, Y, \Phi(X, Y)}\rangle$ is a $\mathrm{no}$-instance, there exists an assignment $\varphi_Y$ such that $\Phi(\varphi_X, \varphi_Y) = 0$.
    Let $D$ consist of the $n + m$ literal vertices corresponding to the literals that evaluate to true under assignments $\varphi_X$ and $\varphi_Y$.
    Then, $D$ is a dominating set of $G-F$: since every vertex in $D$ is incident to no edge in $F$, all vertices in the variable gadgets, as well as all vertices $h_i$, are dominated; since, for each $c_i$, there exists a literal that evaluates to false, $c_i$ is dominated by the corresponding complementary vertex in $D$.

    Therefore, in both cases, we have $\gamma(G-F) = n + m = \gamma(G)$, and hence $b(G) > n$.
\end{proof}

% \begin{corollary}
%   \bondage is $\SigmaTwoP$-complete.
% \end{corollary}

==> intro.tex <==
\section{Introduction}
A dominating set of a graph is a set of vertices such that every vertex outside the set has a neighbor in it. The minimum size of a dominating set is the domination number $\gamma(G)$, a well-studied parameter in graph theory. A natural question is how stable this optimum is under modifications of the graph. In this direction, Fink et al.~\cite{DBLP:journals/dm/FinkJKR90} introduced the \emph{bondage number} $b(G)$, defined as the minimum number of edges whose deletion increases the domination number. The corresponding \bondage problem asks, given a graph $G$ and an integer $d$, whether $b(G)\le d$.

Despite its long history, the precise computational complexity of \bondage has remained unresolved.  
Hu and Xu~\cite{DBLP:journals/jc/HuX12} proved that \bondage is \NP-hard and conjectured that it does not belong to \NP.
Recently, Bakal and Borse~\cite{DBLP:conf/iwoca/BakalB26} showed that even \textsc{1-Bondage} is both NP-hard and coNP-hard, thereby confirming this conjecture under the standard assumption $\NP \neq \coNP$. 
These results demonstrate that \bondage has complexity beyond the usual NP framework, but they do not determine its precise location in the polynomial hierarchy.

In this paper, we first settle this question. We show that, for every fixed
integer $d \ge 1$, $d$-\bondage is $\ThetaTwoP$-complete even on
chordal graphs, where $\ThetaTwoP=P^{\mathrm{NP}[O(\log n)]}$.
Moreover, when the deletion bound is part of the input, we prove that
\bondage is $\SigmaTwoP$-complete. Thus, the fixed-bound and
general versions are complete for $\ThetaTwoP$ and $\SigmaTwoP$,
respectively, giving a precise classification of the classical
\bondage problem.

Having determined the classical complexity of \bondage, we next
ask whether structural restrictions on the input graph can restore
tractability.  We study this question from the viewpoint of parameterized
complexity. 
We obtain fixed-parameter tractability under
several structural parameters, including treewidth. In contrast,
parameterization by the domination number $\gamma(G)$ is \paraNP-hard,
thereby resolving the \W[1]-hardness conjecture of Bakal and Borse~\cite{DBLP:conf/iwoca/BakalB26}
in a stronger form. We further show that W[1]-hardness persists even when
the deletion bound is fixed to $d=1$. Figure~\ref{fig:overview} and
Section~\ref{sec:ourcontribution} give a detailed overview of our results.

\subsection{Related work}
Domination is a classical and extensively studied topic in graph theory, and the
minimum dominating set problem is one of the standard \NP-hard graph
optimization problems.  Numerous variants of domination and their
algorithmic and structural properties have been studied extensively~\cite{DBLP:books/daglib/0093827}.

The bondage number was introduced by Fink et al.~\cite{DBLP:journals/dm/FinkJKR90}
in 1990 as a measure of the vulnerability of domination under edge
failures. Their original work established bounds on the bondage number
and determined its exact value for several basic graph classes, including
complete graphs, paths, cycles, and complete multipartite graphs.
Since then, the bondage number has been studied extensively from a
graph-theoretic viewpoint, with particular attention to upper and lower
bounds, exact values for special graph classes, planar graphs, and various
generalizations.  We refer to the survey of Xu~\cite{xu2013bondage} for an
overview of these developments.

From the algorithmic viewpoint, the picture has been much less complete.
A linear-time algorithm is known for trees, whereas Hu and Xu~\cite{DBLP:journals/jc/HuX12}
show that \bondage is NP-hard on general graphs and conjecture that it
does not belong to NP. NP-hardness is also known for bipartite graphs~\cite{DBLP:journals/tcs/HuS14}.
Bouquet~\cite{DBLP:journals/corr/abs-2107-11216} showed that even $1$-\bondage is NP-hard on
3-regular planar graphs. Together with the general bound
$b(G)\le 2\overline d(G)-1$~\cite{DBLP:journals/dm/HartnellR99}, this immediately implies \paraNP-hardness
when parameterized by the bondage number $b(G)$ itself.
Bakal and Borse~\cite{DBLP:conf/iwoca/BakalB26} have shown that even
1-\bondage is both \NP-hard and \coNP-hard, already on split graphs.

Bakal and Borse~\cite{DBLP:conf/iwoca/BakalB26} also study the
parameterized complexity of \bondage.  Since it is \NP-hard already
for $d=1$, parameterization by the solution size $d$ alone does not even
yield an \XP{} algorithm unless $\P=\NP$.  On the positive side, for every
fixed $d$, they show that \dbondage is fixed-parameter tractable when
parameterized by clique-width.  Their brute-force argument further gives
an \XP{} algorithm for the combined parameter $d+\operatorname{cw}(G)$,
and they leave open whether this combined parameter yields an \FPT{}
algorithm.  They also conjecture that \bondage is \W[1]-hard when
parameterized by the domination number $\gamma(G)$.  
%In this paper, we confirm the latter conjecture, even for $d=1$, and investigate tractability under several other structural parameters.

Parameterized algorithms for domination problems are often developed
using structural graph parameters such as treewidth.  For
\bondage, however, tractability does not follow immediately
from standard techniques for \textsc{Dominating Set}.  The problem asks
whether there exists an edge set $F$ such that
$\gamma(G-F)>\gamma(G)$, and thus combines the choice of a graph
modification with a comparison of two optimum values.  In particular,
this formulation does not appear to be an immediate consequence of
standard MSO-based meta-theorems for bounded-treewidth  and
bounded-clique-width graphs~\cite{DBLP:journals/iandc/Courcelle90,DBLP:journals/mst/CourcelleMR00}.  This
motivates a direct study of the parameterized complexity of
\bondage under natural structural parameters.

\bondage is closely related to blocker and interdiction problems.
Mahdavi Pajouh et al.~\cite{DBLP:journals/eor/PajouhWBP15} study the minimum edge
blocker dominating set problem, which seeks a minimum set of edges
whose deletion raises the domination value to a prescribed threshold.
More generally, blocker problems for graph parameters have been studied
extensively~\cite{DBLP:journals/gc/BazganBPR15}. Very recently, Gr{\"u}ne and Wulf~\cite{DBLP:journals/tcs/GruneW26} established
$\SigmaTwoP$-completeness for a general minimum-cardinality
interdiction version of \textsc{Dominating Set}.
Their interdiction model forbids selected vertices from being used
in a solution, rather than deleting them from the graph.
As they explicitly note, these two notions do not coincide in general
for vertex- and edge-deletion problems.

\subsection{Our contributions}\label{sec:ourcontribution}
\begin{figure}[t]
\centering
\begin{minipage}[t]{0.48\textwidth}
\centering
\resizebox{\linewidth}{!}{%
\begin{tikzpicture}[
  >=Latex,
  class/.style={
    draw,
    rounded corners,
    minimum width=22mm,
    minimum height=8mm,
    align=center
  },
  result/.style={
    draw,
    rounded corners,
    thick,
    fill=blue!10,
    minimum width=31mm,
    minimum height=10mm,
    align=center
  },
  every node/.style={font=\small}
]

% Level 0
\node[class] (p) at (0,0) {$\P$};

% Level 1
\node[class] (np)   at (-2.6,1.5) {\NP};
\node[class] (conp) at ( 2.6,1.5) {\coNP};

% Classes between the first and second levels
\node[result] (theta) at ($(np)!0.5!(conp)+(0,1.4)$)
  {$\ThetaTwoP$\\[-1mm]
   {\scriptsize fixed $d$: complete}};

\node[class] (delta) at ($(theta)+(0,1.35)$)
  {$\DeltaTwoP=\P^{\NP}$};

% Second level
\node[result] (sigma) at ($(np)+(0,4.2)$)
  {$\SigmaTwoP$\\[-1mm]
   {\scriptsize general $d$: complete}};

\node[class] (pi) at ($(conp)+(0,4.2)$)
  {$\PiTwoP$};

% Inclusion arrows
\draw[->] (p) -- (np);
\draw[->] (p) -- (conp);

\draw[->] (np) -- (theta);
\draw[->] (conp) -- (theta);
\draw[->] (np) -- (sigma);
\draw[->] (conp) -- (pi);

\draw[->] (theta) -- (delta);

\draw[->] (delta) -- (sigma);
\draw[->] (delta) -- (pi);

% Optional frame for the second level
\node[
  draw,
  dashed,
  rounded corners,
  fit=(theta)(delta)(sigma)(pi),
  inner xsep=3mm,
  inner ysep=2mm,
  label=above:{\small Second level of the polynomial hierarchy}
] {};
\end{tikzpicture}
}
\caption*{(a) Classical complexity}
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\textwidth}
\centering
\resizebox{\linewidth}{!}{%
\begin{tikzpicture}[
  >=Latex,
   every node/.style={font=\Large},
   par/.style={
    draw,
    rounded corners,
    minimum width=23mm,
    minimum height=7mm,
    align=center
  },
  aux/.style={
    draw,
    rounded corners,
    dashed,
    minimum width=20mm,
    minimum height=7mm,
    align=center
  },
  ours/.style={
  draw=blue!70!black,
  very thick,
  fill=blue!8
  },
  rel/.style={->, thick},
  strata/.style={gray!55}
]

% ------------------------------------------------
% horizontal strata
% ------------------------------------------------
\draw[strata] (-3.6,6.5) -- (3.6,6.5);
\draw[strata] (-3.6,4.00) -- (3.6,4.00);
\draw[strata] (-3.6,2.05) -- (3.6,2.05);

\node[anchor=west,font=\Large\bfseries] at (-6.7,7.50)
  {\paraNP-hard};
\node[anchor=west,font=\Large\bfseries] at (-6.7,5.00)
  {\W[1]-hard};
\node[anchor=west,font=\Large\bfseries] at (-6.7,3.00)
  {\XP};
\node[anchor=west,font=\Large\bfseries] at (-6.7,1.00)
  {\FPT};

% ------------------------------------------------
% paraNP-hard layer
% ------------------------------------------------
\node[par] (d)     at (-1.5,9.10) {$d$};
\node[par,ours] (gamma) at ( 1.0,9.10) {$\gamma(G)$};
\node[par] (b) at (2.9,7.3) {$b(G)$};

\node[
  right,
  font=\normalsize,
  align=left,
  draw=blue!70!black,
  densely dashed,
  rounded corners,
  fill=blue!8,
  inner xsep=4pt,
  inner ysep=2pt
]
at (0.9,8.0)
{$b(G)\le 4\,\operatorname{tw}(G)-2$};

% ------------------------------------------------
% W[1]-hard layer
% ------------------------------------------------
\node[par,ours] (gammad) at (0.0,5.00) {$\gamma(G)+d$};

\node[font=\normalsize,anchor=west]
  at (-1.5,4.40) {hard even for $d=1$};

% ------------------------------------------------
% open layer
% ------------------------------------------------
\node[par] (cwd) at (-1.5,3.00)
  {$\operatorname{cw}(G)+d$};

% ------------------------------------------------
% FPT layer
% ------------------------------------------------
\node[par,ours] (nd)  at (-2.7,1.00)
  {$\operatorname{nd}(G)+d$};

\node[par,ours] (cvd) at ( 0.0,1.00)
  {$\operatorname{cvd}(G)+d$};

\node[par,ours] (tw)  at ( 2.9,1.00)
  {$\operatorname{tw}(G)$};

% ------------------------------------------------
% parameter dominance:
% bounded lower parameter => bounded upper parameter
% ------------------------------------------------
\draw[rel] (gammad) -- (gamma);
\draw[rel] (gammad) -- (d);

\draw[rel] (cwd) -- (d);
\draw[rel] (nd) -- (cwd);
\draw[rel] (cvd) -- (cwd);

% ------------------------------------------------
% structural side relation
% ------------------------------------------------

\draw[->, thick, blue!70!black] (tw) -- (b);

\end{tikzpicture}
}
\caption*{(b) Parameterized complexity}
\end{minipage}

\caption{Overview of our results. Results established in this paper are
highlighted; dashed highlighting denotes a structural relation.}
\label{fig:overview}
\end{figure}

Figure~\ref{fig:overview} summarizes the complexity landscape of
\bondage, including both previously known results and the results
established in this paper. Our main contributions are as follows.

\begin{itemize}
\item
We determine the classical complexity of \bondage within the second
level of the polynomial hierarchy. For every fixed integer $d\ge 1$,
$d$-\bondage is $\ThetaTwoP$-complete, even on chordal graphs.
When $d$ is part of the input, \bondage is $\SigmaTwoP$-complete. 
Thus, the long-standing question of whether \bondage lies beyond NP is resolved up to standard complexity assumptions. (Section~\ref{sec:ph})

\item
On the tractability side, we develop a treewidth DP that tracks
the increase of partial domination optima under edge deletions, yielding
FPT for $\tw(G)+d$. We further prove the structural bound
$b(G)\le 4\tw(G)-2$ for graphs without isolated vertices, which yields
FPT parameterized by $\tw(G)$ alone. We also obtain \FPT{} algorithms for
$\nd(G)+d$ and $\cvd(G)+d$. 
%On the tractability side, we show that \bondage is fixed-parameter tractable when parameterized by $\operatorname{tw}(G)$ alone.  We also obtain FPT algorithms for the combined parameters  $\operatorname{nd}(G)+d$ and $\operatorname{cvd}(G)+d$. 
%In particular, we establish the structural bound $b(G)\le 4\operatorname{tw}(G)-2$ for graphs without isolated vertices. 
(Section~\ref{sec:fpt})

\item
On the intractability side, we show that parameterization by the domination number $\gamma(G)$ does not yield tractability, though \bondage is polynomial-time solvable when $\gamma(G)=1$.
More precisely, we show that \bondage is \paraNP-hard when parameterized by $\gamma(G)$, already for split graphs with $\gamma(G)=2$, thereby settling the \W[1]-hardness conjecture of Bakal and Borse~\cite{DBLP:conf/iwoca/BakalB26}  in a stronger form. 
We further show that \W[1]-hardness persists even when the deletion bound is fixed to $d=1$. (Section \ref{sec:parahard})
\end{itemize}

%\medskip
%
%The remainder of this paper is organized as follows. Section~\ref{sec:pre} introduces the notation and basic definitions used throughout the paper. Section~3 determines the classical complexity of \bondage within the second level of the polynomial hierarchy. Section~4 presents our fixed-parameter tractability results under several structural parameters. Section~5 establishes the corresponding intractability results for parameterization by the domination number. Finally, Section~6 concludes with several open questions and directions for further research.

==> parameterized-intractability.tex <==
%\section{Parameterized intractability}\label{sec:parahard}
\section{Hardness with respect to the domination number}\label{sec:parahard}
\subsection{\paraNP-hardness}
%\subsection{\paraNP-hardness parameterized by the domination number.}
Bakal and Borse~\cite{DBLP:conf/iwoca/BakalB26} mentioned \bondage parameterized by domination number $\gamma(G)$ as a natural direction distinct from clique-width.
They conjectured that \bondage is $\W[1]$-hard parameterized by $\gamma(G)$.

%We first investigate the complexity of \bondage for the smallest values of the domination number.
%We show that \bondage can be solved in polynomial time when $\gamma(G) = 1$, whereas it becomes \NP-hard already when $\gamma(G) = 2$, even on split graphs.
It is known that \bondage is solvable in polynomial time when $\gamma(G) = 1$~\cite[Lemma 49]{xu2013bondage}. 
In contrast, we show that it becomes \NP-hard already when $\gamma(G) = 2$, even on split graphs, which implies that  
\bondage is \paraNP-hard when parameterized by $\gamma(G)$.
We then complement this result by showing that the conjectured $\W[1]$-hardness persists even under the additional restriction $d = 1$.

%
% 過去の文献で言及しているものがあったためコメントアウト
% 
%We begin with the polynomial-time solvable case.
%
%\begin{theorem}
%    \bondage on graphs with $\gamma(G) = 1$ can be solved in polynomial time.
%\end{theorem}
%\begin{proof}
%    Since $\gamma(G) = 1$, $G$ has at least one universal vertex.
%    Let $U = \{u \in V(G) \mid \text{$u$ is a universal vertex}\}$ be the set of all universal vertices of $G$.
    
%    For every edge set $F \subseteq E(G)$, $\gamma(G-F) > 1$ if and only if $G-F$ has no universal vertex, namely every vertex of $U$ is not a universal vertex in $G-F$.
%    Equivalently, $F$ must contain an edge incident with each vertex of $U$.
    
%    Note that $U$ induces a clique in $G$.

%    We first show that $b(G) \leq \left\lceil{\frac{|U|}{2}}\right\rceil$.
%    Since $G[U]$ is a clique, we can choose an edge set $F \subseteq E(G)$ of size $\left\lceil{\frac{|U|}{2}}\right\rceil$ such that every vertex in $U$ is incident with an edge of $F$.
%    (If $|U| = 1$, choose any edge incident with the unique vertex in $U$.)
%    Then no vertex in $U$ is universal in $G-F$.
%    Thus, $\gamma(G-F) > 1 = \gamma(G)$, and hence $b(G) \leq \left\lceil{\frac{|U|}{2}}\right\rceil$.

%    Conversely, let $F \subseteq E(G)$ such that $\gamma(G-F) > \gamma(G)$. 
%    Then $G-F$ has no universal vertex.
%    Thus, for every $u \in U$, at least one edge of $F$ must be incident with $u$.
%    Since each edge is incident with at most two vertices of $U$, at least $\left\lceil{\frac{|U|}{2}}\right\rceil$ edges are required to cover all vertices of $U$.
%    Therefore, $b(G) \geq |F| \geq \left\lceil{\frac{|U|}{2}}\right\rceil$.
%
%    Thus, $b(G) = \left\lceil{\frac{|U|}{2}}\right\rceil$.

%    The set $U$ can be found by checking which vertices have degree $|V(G)|-1$.
%    Moreover, since $G[U]$ is a clique, the required edge set can be constructed simply by pairing vertices of $U$ (and handling one unmatched vertex when $|U|$ is odd).
%    Hence, both $b(G)$ and a minimum bondage set can be computed in polynomial time.
%\end{proof}

\begin{theorem}
    \bondage is \NP-hard even when the graph $G$ is restricted to split graphs with $\gamma(G) = 2$, and hence \paraNP-hard parameterized by $\gamma(G)$.
\end{theorem}
\begin{proof}
    We prove \NP-hardness by a reduction from \VC. 
    Let $\langle{H, \ell}\rangle$ be an instance of \VC.
    We may assume that $|E(H)| \geq 1$.

    We construct an instance $\langle{G, d}\rangle$ of \bondage from $\langle{H, \ell}\rangle$.
    First, we construct a graph $G$ as follows (see \Cref{fig:paranp-split}):
    \begin{enumerate}
        \item For each edge $e \in E(H)$, add two vertices $x_e^1$ and $x_e^2$.
            Let $X$ denote the set of all such vertices.
        \item Add a vertex $s$, and make $X \cup \{s\}$ a clique.
        \item For each vertex $v \in V(H)$, add a vertex $a_v$.
        Make $a_v$ adjacent to $s$ and to $x_e^i$ for each $i \in \{1,2\}$ and every edge $e$ that is not incident to $v$.
        \item For every pair of distinct vertices $x, y \in X$, add a vertex $b_{x, y}$, and make it adjacent to $s$ and to every vertex of $X \setminus \{x, y\}$, where $b_{x,y} = b_{y,x}$.
        \item Add two vertices $p$ and $q$, each adjacent to every vertex in $X$.
    \end{enumerate}
    \begin{figure}[htbp]
      \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[page=1]{images/paranp-split.pdf}
      \end{subfigure}
      \caption{Illustration of the construction in the reduction from \VC\ to \bondage.}
      \label{fig:paranp-split}
    \end{figure}

    Finally, set $d = \ell$.
    This completes the construction.
    The graph is clearly a split graph, with clique $X \cup \{s\}$.

    \begin{claim}\label{claim:paranp:dominating-set}
        We have $\gamma(G) = 2$.
        Moreover, the minimum dominating sets are exactly the sets $\{x, s\}$ with $x \in X$.
    \end{claim}
    \begin{proof}
        For every $x \in X$, the set $\{x, s\}$ is a dominating set of $G$, since $s$ dominates every vertex except $p$ and $q$, both of which are dominated by $x$.
        Since $G$ has no universal vertex, we have $\gamma(G) \geq 2$.
        Therefore, $\gamma(G) = 2$.

        Conversely, let $D$ be a dominating set of size $2$.
        Since $p$ and $q$ are nonadjacent and have neighbors only in $X$, we have $D \cap X \neq \emptyset$.
        Thus, $D$ contains some vertex $x_e^i$, where $e = \{u, v\} \in E(H)$ and $i \in \{1, 2\}$.
        Write $D = \{x_e^i, w\}$ for some $w \in V(G)$.
        Since neither $a_u$ nor $a_v$ is adjacent to $x_e^i$, $w$ must dominate both $a_u$ and $a_v$.
        This implies that $w \in X \cup \{s\}$.
        If $w \in X$, then the vertex $b_{x_e^i, w}$ is not dominated by $D$.
        Hence, $w = s$, completing the proof.
    \end{proof}

    \begin{claim}\label{claim:paranp:upper_bound}
        $b(G) \leq \tau(H)$.
    \end{claim}
    \begin{proof}
        Let $C \subseteq V(H)$ be a minimum vertex cover of $H$.
        Define $F = \{\{s, a_v\} \mid v \in C\}$.
        Clearly, $|F| = \tau(H) = |C|$.
        We show that $\gamma(G - F) > 2 = \gamma(G)$.
        
        Let $D \subseteq V(G)$ be a minimum dominating set of $G$.
        By \Cref{claim:paranp:dominating-set}, we have $D = \{x_e^j, s\}$, where $e = \{u, v\} \in E(H)$.
        Since $C$ is a vertex cover, at least one endpoint of $e$ belongs to $C$.
        Without loss of generality, let $u \in C$.
        Since $a_u$ is not adjacent to $x_e^j$, we have $N_G(a_u) \cap D = \{s\}$.
        Since $\{s, a_u\} \in F$, the vertex $a_u$ is not dominated by $D$ in $G-F$.
        Thus, no minimum dominating set of $G$ is a dominating set of $G-F$.
        Therefore, $G-F$ has no dominating set of size $2$, and hence $\gamma(G-F) > 2 = \gamma(G)$.
        Consequently, $b(G) \leq |F| = \tau(H)$.
    \end{proof}
    \begin{claim}\label{claim:paranp:lower_bound}
        $b(G) \geq \tau(H)$.
    \end{claim}
    \begin{proof}
        Let $F \subseteq E(G)$ be an edge set such that $\gamma(G-F) > \gamma(G)$.
        Define $C_F = \{v \in V(H) \mid \{s, a_v\} \in F\}$, $F_0 = F \setminus \{\{s, a_v\} \mid v \in V(H)\}$, and $U = \{e \in E(H) \mid e \cap C_F = \emptyset\}$.
        Thus, $U$ is the set of edges of $H$ not covered by $C_F$.

        Let $B$ consist of all vertices in $X$ incident to an edge of $F_0$, together with both $x$ and $y$ for every pair of distinct vertices $x,y \in X$ such that $\{s,b_{x,y}\} \in F_0$.
        Formally, $B = \{x \in X \mid \exists f \in F_0,\ x \in f\} \cup \bigcup_{\{s,b_{x,y}\} \in F_0} \{x,y\}$.
        Since each edge in $F_0$ contributes at most two vertices to $B$, we have $|B| \leq 2|F_0|$.

        We claim that both $x_e^1$ and $x_e^2$ belong to $B$ for every $e \in U$.
        Suppose otherwise, that is, $x = x_e^i \notin B$ for some $e = \{u,v\} \in U$ and $i \in \{1,2\}$.
        By construction, the only vertices nonadjacent to $x$ are $a_u$, $a_v$, and $b_{x,y}$ for $y \in X \setminus \{x\}$.
        Since $x \notin B$, no edge incident to $x$ is deleted, and $\{s,b_{x,y}\} \notin F$ for every $y \in X \setminus \{x\}$.
        Moreover, since $e \in U$, neither $\{s,a_u\}$ nor $\{s,a_v\}$ belongs to $F$.
        Consequently, $\{s,x\}$ is a dominating set of $G-F$ of size two, contradicting $\gamma(G-F) > \gamma(G) = 2$.
        Hence, $\{x_e^1,x_e^2 \mid e \in U\} \subseteq B$.
        Since all these vertices are distinct, we have $2|U| \leq |B| \leq 2|F_0|$, which implies $|U| \leq |F_0|$.

        For each $e \in U$, choose an endpoint $v_e \in e$ and define $C = C_F \cup \{v_e \mid e \in U\}$.
        Then $C$ is a vertex cover of $H$, since every edge in $U$ is covered by its chosen endpoint $v_e$, while every edge not in $U$ has an endpoint in $C_F$.
        Moreover, $|C| \leq |C_F| + |U| \leq |C_F| + |F_0| = |F|$.
        Thus, $\tau(H) \leq |F|$.
        Since $F$ was an arbitrary edge set satisfying $\gamma(G-F) > \gamma(G)$, we conclude that $b(G) \geq \tau(H)$.
        This proves the claim.
    \end{proof}

    By \Cref{claim:paranp:upper_bound,claim:paranp:lower_bound}, $b(G) = \tau(H)$.
    Hence, the instance $\langle{H, \ell}\rangle$ of \VC is a yes-instance if and only if the constructed instance $\langle{G, d}\rangle$ of \bondage is a yes-instance.
    This proves the theorem.
\end{proof}

% \begin{theorem}
%  \bondage is \NP-hard even on bipartite graphs whose domination number is $3$.
% \end{theorem}
% \begin{proof}
%     We prove the \NP-hardness by a reduction from \VC.
%     It is known that \VC is \NP-complete even on triangle-free cubic graphs~\cite{Uehara1996NPComplete}.

%     Let $\langle{H, \ell}\rangle$ be an instance of \VC, where $H$ is a triangle-free cubic graph.
%     We may assume that $\ell \leq |V(H)|$.
%     Since $H$ is a cubic graph, $|V(H)| \geq 4$.

%     \paragraph{construction.}
%     We now construct an instance $\langle{G, d}\rangle$ of \bondage from $langle{H, \ell}\rangle$.
%     First, we construct graph $G$ as follows (see \Cref{fig:paranp}):
%     \begin{itemize}
%         \item For every vertex $v \in V(H)$, add a vertex $a_v$.
%         \item For every vertex $v \in V(H)$, add a vertex $b_v$.
%         \item For every pair $u, v \in V(H)$ of vertices, if $u = v$ or $\{u, v\} \notin E(H)$, add an edge $\{a_u, b_v\}$.
%         \item For every pair $\{u, v\} \notin E(H) \quad (u \neq v)$ of nonadjacent vertices, add two vertices $w_{u,v}^1$ and $w_{u, v}^2$.
%         \item For every pair $\{u, v\} \notin E(H) \quad (u \neq v)$ and a vertex $x \in V(H)$, if $x \neq u$ and $x \neq v$, add edges $\{a_x, w_{u,v}^1\}$ and $\{a_x, w_{u,v}^2$.
%         \item For every $1 \leq i \leq \ell + 1$, add a vertex $s_i$.
%         \item For every $v \in V(H)$ and $1 \leq i \leq \ell+1$, add an edge $\{a_v, s_i\}$.
%     \end{itemize}
%     Let $A = \{a_v \mid v \in V(H)\}$, $B = \{b_v \mid v \in V(H)\}$, $W = \{w_{u,v}^1, w_{u,v}^2 \mid \{u,v\} \notin E(H)\}$ and $S = \{s_i \mid 1 \leq i \leq \ell + 1\}$.
%     \begin{figure}[htbp]
%       \centering
    
%       % Top: original graph
%       \begin{subfigure}{0.40\textwidth}
%         \centering
%         \includegraphics[page=1,width=\linewidth]{images/paranp.pdf}
%         \caption{The original graph $H$.}
%         \label{fig:reduction-original}
%       \end{subfigure}
    
%       \vspace{1em}
    
%       % Bottom left
%       \begin{subfigure}{0.31\textwidth}
%         \centering
%         \includegraphics[page=2,width=\linewidth]{images/paranp.pdf}
%         \caption{Edges between $A$ and $B$.}
%         \label{fig:reduction-ab}
%       \end{subfigure}
%       \hfill
%       % Bottom center
%       \begin{subfigure}{0.31\textwidth}
%         \centering
%         \includegraphics[page=3,width=\linewidth]{images/paranp.pdf}
%         \caption{Edges between $A$ and $W$.}
%         \label{fig:reduction-aw}
%       \end{subfigure}
%       \hfill
%       % Bottom right
%       \begin{subfigure}{0.31\textwidth}
%         \centering
%         \includegraphics[page=4,width=\linewidth]{images/paranp.pdf}
%         \caption{Edges between $A$ and $S$.}
%         \label{fig:reduction-as}
%       \end{subfigure}
    
%       \caption{
%         Illustration of the construction of $G$ from $H$.
%         For clarity, we focus on four vertices $u,v_1,v_2,v_3 \in V(H)$
%         such that $\{u,v_i\}\in E(H)$ for each $i\in\{1,2,3\}$.
%         The figures show only the part of G corresponding to these four vertices.
%         The top figure shows the subgraph of $H$ induced by these vertices,
%         while the three bottom figures illustrate the corresponding parts
%         of the constructed graph $G$, showing the adjacencies between
%         $A$ and $B$, between $A$ and $W$, and between $A$ and $S$,
%         respectively.
%       }
%       \label{fig:paranp}
%     \end{figure}
%     Finally, we set $d = \ell$.
%     This completes the construction of the instance.

%     We first show that $G$ is a bipartite graph and the domination number $\gamma(G)$ is a constant.

%     \begin{claim}
%         The graph $G$ is a bipartite graph.
%     \end{claim}
%     \begin{proof}
%         The sets $A, B, W, S$ are the partitions of $V(G)$.
%         Moreover, the edges of $G$ is only between a vertex of $A$ and a vertex of $B \cup W \cup S$.
%         Thus, the graph $G$ is a bipartite graph with a bipartition $A$ and $B \cup W \cup S$.
%     \end{proof}

%     \begin{claim}
%         We have $\gamma(G) = 3$.
%         Moreover, a set $D \subseteq V(G)$ is a minimum dominating set of $G$ if and only if $D = \{a_u, a_v, s_i\}$ for $\{u, v\} \in E(H)$ and $1 \leq i \leq \ell + 1$.
%     \end{claim}
%     \begin{proof}
%         First, we prove that $\gamma(G) \leq 3$.
%         Let $1 \leq i \leq \ell + 1$ and $\{u, v\} \in E(H)$.
%         Let $D = \{a_u, a_v, s_i\}$.
%         We claim that $D$ is a dominating set of $G$.

%         Since $A$ and $S$ are completely adjacent, the set $D$ dominates the vertices of both of $A$ and $S$

%         Suppose that $B$ is not dominated by $D$, that is there is a vertex $b_x \in B$ that is not adjacent to both of $a_u$ and $a_v$.
%         By construction, we have $u \neq x \land \{a_u, x\} \in E(H)$ and $v \neq x \land \{a_v, x\} \in E(H)$.
%         Since $u$ and $v$ are adjacent, the vertices $\{u, v, x\}$ forms a triangle in $H$, a contradiction to that $H$ is a triangle-free graph.

%         Finally, we show that $D$ dominates the vertices of $W$.
%         Let $w_{x,y}^j \in W$ where $\{x, y\} \notin E(H)$.
%         Since $\{u, v\} \in E(H)$, we have $\{u, v\} \neq \{x, y\}$.
%         If $u \neq x$ and $u \neq y$, the vertex $a_u$ is adjacent to $w_{x,y}^j$, and thus, the vertex $w_{x,y}^j$ is dominated.
%         It holds true that in the same way if we change $u$ and $v$.
%         Thus, every vertex of $W$ is dominate by $D$.

%         Therefore, the set $D$ is a dominating set of $G$, and thus, we have $\gamma(G) \leq 3$.

%         Now we prove that $\gamma(G) \geq 3$.
%         Let $D' \subseteq V(G)$ is a dominating set of $G$.
%         By above, we may assume that $|D| \leq 3$.
%     \end{proof}
    
% \end{proof}

\subsection{$\W[1]$-hardness for $d=1$}
%\subsection{$\W[1]$-hardness parameterized by the domination number even for $d=1$.}

%Our reduction is inspired by the reduction in~\cite{DBLP:books/sp/CyganFKLMPPS15}.
Our reduction adapts the standard reduction from \textsc{Multicolored Independent Set} to \textsc{Dominating Set} (see, e.g.,~\cite[Theorem~13.9]{DBLP:books/sp/CyganFKLMPPS15}).

\begin{theorem}
    \bondage is $\W[1]$-hard parameterized by $\gamma(G)$ even when restricted to $d = 1$.
\end{theorem}
\begin{proof}
    We give a parameterized reduction from \textsc{Multicolored Independent Set}.
    Given a graph $G$ whose vertices are partitioned into $k$ color classes, the problem asks whether $G$ has an independent set containing exactly one vertex from each color class.
    It is known that \textsc{Multicolored Independent Set} is $\W[1]$-hard parameterized by the number $k$ of color classes~\cite{DBLP:series/mcs/DowneyF99}.
    Let $\langle{G, k, (V_1, \dots, V_k)}\rangle$ be an instance, where $V_1, \dots, V_k$ are the color classes.
    We may assume that $|V_i| \geq 2$ for every $i$: an empty color class makes the instance a no-instance, and a singleton color class can be enlarged by duplicating its unique vertex without changing the answer.

    We first add two vertices $a$ and $b$ such that $a$ is isolated and $b$ is adjacent to every vertex of $G$, and set $V_{k+1} = \{a, b\}$.
    Let the resulting graph be $G'$.
    Clearly, this preprocessing preserves the existence of a multicolored independent set.

    We construct a graph $H$ from $G'$ as follows (see \Cref{fig:w1-hard}).
    \begin{enumerate}
        \item Add all vertices of $G'$ to $H$.
        \item For every $1 \leq i \leq k+1$, make $V_i$ a clique in $H$.
        \item For every edge $e = \{u, v\} \in E(G')$, where $u \in V_i$ and $v \in V_j$ with $i \neq j$, add a new vertex $w_e$ adjacent to every vertex in $(V_i \cup V_j) \setminus \{u, v\}$.
        \item For every $1 \leq i \leq k+1$, add two new vertices $x_i$ and $y_i$, each adjacent to every vertex in $V_i$.
        \item Add a new vertex $z$ adjacent to every vertex of $G'$ and to every vertex $w_e$ for $e \in E(G')$.
    \end{enumerate}
    This completes the construction of $H$.
    Finally, set $d = 1$.

    \begin{figure}[htbp]
        \centering
        \includegraphics{images/w1-hard.pdf}
        \caption{The graph $H$ in our construction. The illustration is adapted from the presentation of the corresponding multicolored gadget in~\cite{DBLP:books/sp/CyganFKLMPPS15}. The set $V_i \cup \{x_i, y_i\}$ induces a clique minus the edge $\{x_i, y_i\}$. If an edge $e$ connects $u \in V_i$ and $v \in V_j$, then we add a vertex $w_e$ adjacent to every vertex in $(V_i \cup V_j) \setminus \{u, v\}$. We also add a vertex $z$ adjacent to all vertices of $G'$ and to every vertex $w_e$, but to neither $x_i$ nor $y_i$.}
        \label{fig:w1-hard}
    \end{figure}

    \begin{claim}\label{claim:w1-hard:2}
        $k+1 \leq \gamma(H) \leq k+2$.
    \end{claim}
    \begin{proof}
        Let $D$ be a minimum dominating set of $H$.
        For every $1 \leq i \leq k+1$, the vertices $x_i$ and $y_i$ are adjacent only to the vertices in $V_i$.
        The set $D$ must contain at least one vertex from $V_i \cup \{x_i, y_i\}$ to dominate both $x_i$ and $y_i$.
        Since this holds for every $1 \leq i \leq k+1$, we obtain $|D|\geq k+1$.
        Therefore, $\gamma(H)\geq k+1$.

        To prove the upper bound, choose an arbitrary vertex $v_i\in V_i$ for every $1 \leq i \leq k+1$, and let $D'=\{v_i\mid 1 \leq i \leq k+1\}\cup\{z\}$.
        For every $1 \leq i \leq k+1$, the vertex $v_i$ dominates every vertex in $V_i$, since $V_i$ is a clique.
        Moreover, $v_i$ dominates both $x_i$ and $y_i$.
        Every vertex $w_e$, where $e\in E(G')$, is dominated by $z$, and $z$ dominates itself.
        Thus, $D'$ is a dominating set of $H$.
        Since $|D'|=k+2$, we obtain $\gamma(H) \leq k+2$.
    \end{proof}

    \begin{claim}\label{claim:w1-hard:3}
        $\gamma(H) = k+1$ if and only if the graph $G'$ has an independent set containing exactly one vertex from each of the color classes.
    \end{claim}
    \begin{proof}
        Suppose that $\gamma(H)=k+1$.
        Let $D \subseteq V(H)$ be a dominating set of size $k+1$.
        For every $1 \leq i \leq k+1$, as stated above, the set $D$ must contain at least one vertex from $V_i \cup \{x_i,y_i\}$.
        Since these $k+1$ sets are pairwise disjoint and $|D|=k+1$, the set $D$ contains exactly one vertex from $V_i \cup \{x_i,y_i\}$ for each $1 \leq i \leq k+1$.
        Since $x_i$ and $y_i$ are not adjacent to each other, $D$ must contain a vertex in $V_i$ to dominate both $x_i$ and $y_i$.
        Thus, $D$ consists of vertices $v_i \in V_i$ for $1 \leq i \leq k+1$.
        We now claim that $D$ is an independent set of $G'$.
        Suppose that some $v_i \in D$ and $v_j \in D$, where $i \neq j$, are adjacent in $G'$.
        Then there exists an edge $e=\{v_i,v_j\}\in E(G')$.
        Consider the vertex $w_e$ in $H$.
        Since $w_e$ is adjacent only to the vertices in $(V_i\cup V_j)\setminus\{v_i,v_j\}$ and to $z$, the vertex $w_e$ is not dominated by $D$, a contradiction.
        Thus, no two vertices in $D$ are adjacent in $G'$, and hence $D$ is an independent set of $G'$.
        Moreover, $D$ contains exactly one vertex from each color class.

        Conversely, suppose that $G'$ has an independent set containing exactly one vertex from each color class.
        Let $I$ be such an independent set.
        We show that $I$ is a dominating set of $H$.
        Write $I=\{v_1,\dots,v_k, v_{k+1}\}$, where $v_i\in V_i$.
        For every $1 \leq i \leq k+1$, the vertex $v_i$ dominates every vertex in $V_i \cup \{x_i,y_i\}$. 
        The vertex $v_{k+1}$ dominates $z$.
        Now consider a vertex $w_e$, where $e = \{u, v\} \in E(G')$, $u \in V_i$ and $v \in V_j$ with $i \neq j$.
        Since $I$ is independent in $G'$, we cannot have both $v_i = u$ and $v_j = v$.
        Hence, either $v_i \neq u$ or $v_j \neq v$.
        If $v_i \neq u$, then $v_i$ is adjacent to $w_e$; otherwise, $v_j\neq v$, and $v_j$ is adjacent to $w_e$.
        Thus, every vertex $w_e$ is dominated by $I$.
        Therefore, $I$ is a dominating set of $H$ of size $k+1$.
        Since $\gamma(H)\geq k+1$, we obtain $\gamma(H)=k+1$.
    \end{proof}

    \begin{claim}\label{claim:w1-hard:4}
        $\gamma(H) = k+1$ if and only if $b(H) = 1$.
    \end{claim}
    \begin{proof}
        Suppose first that $\gamma(H) = k+1$.
        Consider the edge $e = \{a,x_{k+1}\}$.
        Suppose that $\gamma(H-e)=k+1$.
        Then there exists a dominating set $D$ of $H-e$ of size $k+1$.
        For every $1 \leq i \leq k+1$, the set $D$ must contain at least one vertex from $V_i \cup \{x_i, y_i\}$.
        Since these $k+1$ sets are pairwise disjoint and $|D|=k+1$, the set $D$ contains exactly one vertex from each of them.
        In $H-e$, the only vertex in $V_{k+1}\cup\{x_{k+1},y_{k+1}\}$ that dominates both $x_{k+1}$ and $y_{k+1}$ is $b$.
        Therefore, $b\in D$.
        The set $D$ is also a dominating set of $H$ of size $k+1$.
        Therefore, by the argument in the forward direction of \Cref{claim:w1-hard:3}, $D$ consists of exactly one vertex from each $V_i$ and is an independent set in $G'$.
        However, $b$ is adjacent in $G'$ to every vertex in $V_1, \dots, V_k$.
        Since $D$ contains $b$ and one vertex from each of $V_1,\dots,V_k$, this is a contradiction.
        Therefore, $\gamma(H-e)>\gamma(H)$, and hence $b(H)=1$.

        Conversely, suppose that $\gamma(H) \neq k+1$.
        By \Cref{claim:w1-hard:2}, $\gamma(H)=k+2$.
        We show that $\gamma(H-f)=k+2$ for every edge $f\in E(H)$.
        By the construction of $H$, every edge $f\in E(H)$ is of one of the following types:
        \begin{itemize}
            \item[(i)] $f$ is an edge between a vertex in $\{x_i, y_i\}$ and a vertex $v \in V_i$.
            \item[(ii)] $f$ is an edge with endpoints $u,v \in V_i$.
            \item[(iii)] $f$ is an edge between a vertex $v \in V_i$ and a vertex $w_e$, where $e \in E(G')$.
            \item[(iv)] $f$ is an edge between $z$ and a vertex $v \in V_i$.
            \item[(v)] $f=\{z,w_e\}$ for some edge $e = \{u,v\} \in E(G')$, where $u \in V_i$ and $v \in V_j$.
        \end{itemize}
        For each $1\leq i\leq k+1$, choose a vertex $v_i\in V_i$, and let $D_f = \{v_i \mid 1 \leq i \leq k+1\} \cup \{z\}$.
        We choose the vertices $v_i$ depending on the type of $f$.
        In Case (i), where $f$ joins a vertex in $\{x_i,y_i\}$ and a vertex $v \in V_i$, choose $v_i \in V_i \setminus \{v\}$.
        Such a choice is possible because $|V_i| \geq 2$.
        In Cases (ii), (iii) and (iv), choose every $v_i$ arbitrarily.
        In Case (v), where $f = \{z,w_e\}$ and $e = \{u,v\}$ with $u \in V_i$ and $v \in V_j$, choose $v_i \in V_i \setminus \{u\}$.
        Again, such a choice is possible because $|V_i| \geq 2$.
        In every case, $D_f$ is a dominating set of $H-f$ of size $k+2$, and hence $\gamma(H-f) \leq k+2$.
        On the other hand, deleting an edge cannot decrease the domination number, so $\gamma(H-f) \geq \gamma(H) = k+2$.
        Therefore, $\gamma(H-f)=k+2$ for every $f\in E(H)$.
        Thus, deleting any single edge of $H$ does not increase the domination number, and hence $b(H)\neq 1$. 
    \end{proof}

    From \Cref{claim:w1-hard:3,claim:w1-hard:4}, we obtain that $G$ has an independent set containing exactly one vertex from each color class if and only if $b(H) = 1$.
    Moreover, \Cref{claim:w1-hard:2} gives $\gamma(H) \leq k+2$, so the parameter of the constructed instance is bounded by a function of the parameter of the original instance.
    This completes the proof.
\end{proof}

==> parameterized-tractability.tex <==
%\section{Parameterized complexity}
\section{Fixed-Parameter Tractability}\label{sec:fpt}
We next study structural parameters that lead to fixed-parameter
tractability.  We first give an algorithm parameterized by treewidth
alone.  We then consider neighborhood-based parameters, for which the
bounded number of vertices incident with deleted edges allows us to
exploit symmetry among vertices with the same neighborhood.

%\subsection{\bondage parameterized by treewidth.}
\subsection{Treewidth}\label{sec:tw}

We show that \bondage is fixed-parameter tractable parameterized by the treewidth of the input graph.
Our proof proceeds in two steps.
First, given an integer $d$, we give a fixed-parameter algorithm parameterized by $\mathrm{tw}(G)+d$.
We then show that the relevant values of $d$ can be bounded in terms of $\mathrm{tw}(G)$.
This yields fixed-parameter tractability with respect to treewidth alone.

Let $k=\mathrm{tw}(G)$.
We use a nice tree decomposition $T$ of width $k$, rooted at a node $r$, whose root and leaves have empty bags.
We additionally use introduce edge nodes and assume that every edge of $G$ is introduced exactly once.
For each node $t\in V(T)$, let $X_t$ denote its bag.
Let $T_t$ denote the subtree of $T$ rooted at $t$, let $V_t=\bigcup_{s\in V(T_t)} X_s$, and let $E_t$ be the set of edges introduced at nodes of $T_t$.
We write $G_t=(V_t,E_t)$.

Our algorithm builds on the standard dynamic programming (DP) algorithm for \textsc{Dominating Set} over a nice tree decomposition; see~\cite{DBLP:books/sp/CyganFKLMPPS15}.

For each node $t$, consider a coloring $f: X_t \to \{0, \hat{0}, 1\}$.
Let $\mathcal{C}_t = \{0,\hat{0},1\}^{X_t}$ denote the set of all such colorings.
If $X_t = \emptyset$, then $\mathcal{C}_t = \{\emptyset\}$, where $\emptyset$ denotes the unique coloring of the empty bag.
For a node $t$ and a coloring $f$, a vertex set $D \subseteq V_t$ is \textit{compatible} with ($t$, $f$) if
\begin{itemize}
    \item $D \cap X_t = f^{-1}(1)$, and
    \item $D$ dominates every vertex in $V_t \setminus f^{-1}(\hat{0})$ in $G_t$.
\end{itemize}
Thus, a vertex colored $0$ is not contained in the dominating set and must be dominated; a vertex colored $1$ must belong to the dominating set; and a vertex colored $\hat{0}$ does not belong to the dominating set but is not required to be dominated.
For a node $t$ and a coloring $f$, let $c[t, f]$ denote the minimum size of a compatible set with ($t$, $f$) in $G_t$.
If no such $D$ exists, define $c[t, f] = +\infty$.
Then $c[r, \emptyset]$ at the root $r$ is the size of a minimum dominating set of $G$, since $X_r = \emptyset$ and $G_r = G$.

We now show the recursive formulas for the values of $c$ at each type of node.
For a coloring $f$, let $f_{v \to a}$ denote the coloring obtained by assigning color $a$ to $v$ and leaving all other assignments unchanged.
If $v$ is not in the domain of $f$, we extend the domain to include $v$.
We write $f|_X$ for the restriction of $f$ to $X$.

\paragraph{Leaf node.}
Let $t$ be a leaf node.
Since $X_t = \emptyset$, we have $c[t, \emptyset] = 0$.

\paragraph{Introduce vertex node.}
Let t be an introduce vertex node with a child $t'$, where $X_t = X_{t'} \cup \{v\}$ for some $v \notin X_{t'}$.
The vertex $v$ is isolated in $G_t$ and therefore cannot be dominated by any other vertex.
Hence,
\begin{align*}
    c[t, f] = \begin{cases}
                +\infty & \text{when} \quad f(v) = 0\\
                c[t', f|_{X_{t'}}] & \text{when} \quad f(v) = \hat{0} \\
                1 + c[t', f|_{X_{t'}}] & \text{when} \quad f(v) = 1
            \end{cases}
\end{align*}

\paragraph{Introduce edge node.}
Let t be an introduce edge node with child $t'$, where $E_{t} = E_{t'} \cup \{e\}$ with $e = \{u, v\}$ and $u, v \in X_t$.
If $u$ is colored as $1$ and $v$ is colored as $0$, $u$ dominates $v$; thus, we can relax the constraint of $v$ to $\hat{0}$.
The case where $u$ is colored $0$ and $v$ is colored $1$ is symmetric.
Then,
\begin{align*}
    c[t, f] = \begin{cases}
                c[t', f_{v \to \hat{0}}] & \text{when} \quad (f(u), f(v)) = (1, 0)\\
                c[t', f_{u \to \hat{0}}] & \text{when} \quad (f(u), f(v)) = (0, 1)\\
                c[t', f] & \text{otherwise}
            \end{cases}
\end{align*}

\paragraph{Forget node.}
Let t be a forget node with child $t'$, where $X_t = X_{t'} \setminus \{w\}$ for some $w \in X_{t'}$ .
Once a vertex has been forgotten, it cannot be dominated by a vertex introduced later; therefore, it must already be dominated in $G_{t'}$.
Thus,
\begin{align*}
    c[t, f] = \min\{c[t', f_{w \to 1}], c[t', f_{w \to 0}]\}.
\end{align*}

\paragraph{Join node.}
Let $t$ be a join node with children $t_1$ and $t_2$.
Then $X_t = X_{t_1} = X_{t_2}$.
Let $f_1$ and $f_2$ be colorings at $t_1$ and $t_2$, respectively.
We say that ($f_1$, $f_2$) are \textit{consistent} with $f$ if, for every vertex $v \in X_t$, $(f(v), f_1(v), f_2(v)) \in \{(1,1,1), (0,0,\hat{0}),(0,\hat{0},0),(\hat{0},\hat{0},\hat{0})\}$.
If a set $D$ is compatible with ($t$, $f$), then there exist colorings ($f_1$, $f_2$) consistent with $f$ such that $D_1 \coloneqq D\cap V_{t_1}$ and $D_2 \coloneqq D \cap V_{t_2}$ are compatible with $(t_1, f_1)$ and $(t_2, f_2)$, respectively.
Conversely, if ($f_1$, $f_2$) are consistent with $f$ and $D_1, D_2$ are compatible with $(t_1, f_1)$ and $(t_2, f_2)$, respectively, then $D \coloneqq D_1 \cup D_2$ is compatible with ($t$, $f$).
Therefore, we update
\begin{align*}
  c[t, f] = \min_{\substack{(f_1, f_2) \\ \text{consistent with $f$}}}\{c[t_1, f_1] + c[t_2, f_2] - |f^{-1}(1)|\}.
\end{align*}

We next show the DP for \bondage.
We first prove the following lemma.
\begin{lemma}\label{lemma:diff}
  Let $F \subseteq E_t$.
  If there exists a set compatible with ($t$, $f$) in $G_t-F$, then the minimum size of such a set is between $c[t,f]$ and $c[t,f]+|F|$.
\end{lemma}
\begin{proof}
    If there exists $D \subseteq V_t$ that is compatible in $G_t - F$ with $|D| < c[t, f]$, then $D$ is also compatible in $G_t$, a contradiction.
    Thus, the minimum size of a compatible set in $G_t-F$ is at least $c[t,f]$.

    Conversely, let $D \subseteq V_t$ be a compatible set in $G_t$ with $|D| = c[t, f]$.
    Let $U$ be the set of all vertices of $V_t \setminus f^{-1}(\hat{0})$ that are not dominated by $D$ in $G_t - F$.
    We have $U \cap D = \emptyset$ and $|U| \leq |F|$.
    Let $D' \subseteq V_t$ be a compatible set in $G_t - F$.
    For each $v \in U$, choose a vertex $x_v \in D'$ that dominates $v$ in $G_t - F$.
    We have $x_v \notin D$, since otherwise $D$ dominates $v$ in $G_t-F$.
    Hence $x_v \in D' \setminus D$.
    By compatibility, $D \cap X_t = D' \cap X_t = f^{-1}(1)$, so $(D' \setminus D) \cap X_t = \emptyset$.
    Therefore, $D'' = D \cup \{x_v \mid v \in U\}$ is compatible in $G_t - F$ and we have $|D''| \leq |D| + |U| \leq c[t, f] + |F|$.
\end{proof}

\Cref{lemma:diff} shows that deleting at most $d$ edges can increase each finite partial optimum by at most $d$.
Hence, rather than storing the optimum value itself, it suffices to record its difference from the corresponding value in the original graph.

We now introduce a \textit{difference function} $\delta: \mathcal{C}_t \to \{0,1,\dots,d,\infty\}$.
For $F \subseteq E_t$ with $|F| \leq d$, we say that $F$ \textit{realizes} a map $\delta$ if, for every coloring $f$, the following holds: if there exists a set compatible with ($t$, $f$) in $G_t-F$, then the minimum size of such a set is $c[t,f]+\delta(f)$; otherwise, $\delta(f)=+\infty$.
For each node $t$ and map $\delta$, let $\mathrm{DP}[t,\delta]$ be the minimum size of a set $F \subseteq E_t$ with $|F| \leq d$ that realizes $\delta$.
If no such $F$ exists, let $\mathrm{DP}[t,\delta] = +\infty$.
Then, at the root $r$, $b(G) \leq d$ if and only if there exists a difference function $\delta$ such that $\mathrm{DP}[r,\delta] \leq d$ and $\delta(\emptyset) \geq 1$.
We initialize all entries to $+\infty$ before applying the transitions below.

\paragraph{Leaf node.}
Let $t$ be a leaf node.
Since $X_t = \emptyset$ and $E_t = \emptyset$, the only possible edge deletion set is $F = \emptyset$.
Thus, the only realizable state is $\delta_0$, defined by $\delta_0(\emptyset) = 0$.
We initialize $\mathrm{DP}[t,\delta_0] = 0$.

\paragraph{Introduce vertex node.}
Let $t$ be an introduce vertex node with child $t'$, where $X_t = X_{t'} \cup \{v\}$ for some $v \notin X_{t'}$.
No edge is introduced at $t$, so $E_t = E_{t'}$ and the possible edge deletion sets are the same at the two nodes.

Let $\delta'$ be a state at $t'$.
Since $v$ is isolated in $G_t$, it can neither dominate nor be dominated by any other vertex.
Consequently, if $\delta'$ is realized by an edge set $F' \subseteq E_{t'}$, the same set $F = F'$ realizes a parent state whose values are determined by the color of $v$.

For every $\delta'$ with $\mathrm{DP}[t',\delta'] \leq d$, define
\begin{align*}
  \delta(f) = \begin{cases}
    +\infty & \text{if } f(v) = 0, \\
    \delta'(f|_{X_{t'}}) & \text{otherwise,}
  \end{cases}
\end{align*}
and update
\begin{align*}
  \mathrm{DP}[t,\delta] \gets \min\{\mathrm{DP}[t,\delta],\mathrm{DP}[t',\delta']\}.
\end{align*}

\paragraph{Introduce edge node.}
Let $t$ be an introduce edge node with child $t'$ that introduces an edge $e = \{u,v\} \notin E_{t'}$.
Then $X_t = X_{t'}$, $E_t = E_{t'} \cup \{e\}$, and $\mathcal{C}_t = \mathcal{C}_{t'}$.

Let $\delta'$ be a state at $t'$ realized by some $F' \subseteq E_{t'}$.
We distinguish between retaining and deleting $e$.

If $e$ is retained, let $F^{\text{keep}} = F'$.
When $(f(u),f(v)) = (1,0)$, the vertex $u$ dominates $v$.
Thus, for every $D \subseteq V_t$, the set $D$ is compatible with ($t$, $f$) in $G_t-F^{\text{keep}}$ if and only if it is compatible with ($t'$, $f_{v \to \hat{0}}$) in $G_{t'}-F'$.
Therefore, the minimum size of a compatible set in $G_t-F^{\text{keep}}$ is $c[t',f_{v \to \hat{0}}]+\delta'(f_{v \to \hat{0}})$.
The standard DP transition gives $c[t,f] = c[t',f_{v \to \hat{0}}]$, so the corresponding difference is $\delta'(f_{v \to \hat{0}})$ whenever the minimum is finite; otherwise, the difference is $+\infty$.
The case $(f(u),f(v)) = (0,1)$ is symmetric.
In all other cases, introducing $e$ does not change the family of compatible sets.

For every $\delta'$ with $\mathrm{DP}[t',\delta'] \leq d$, define
\begin{align*}
  \delta^{\text{keep}}(f) = \begin{cases}
    \delta'(f_{v \to \hat{0}}) & \text{if } (f(u),f(v)) = (1,0), \\
    \delta'(f_{u \to \hat{0}}) & \text{if } (f(u),f(v)) = (0,1), \\
    \delta'(f) & \text{otherwise.}
  \end{cases}
\end{align*}
Since the number of deleted edges is unchanged, we update
\begin{align*}
  \mathrm{DP}[t,\delta^{\text{keep}}] \gets
  \min\{\mathrm{DP}[t,\delta^{\text{keep}}],\mathrm{DP}[t',\delta']\}.
\end{align*}

If $e$ is deleted, let $F^{\text{delete}} = F' \cup \{e\}$.
Then $G_t-F^{\text{delete}} = G_{t'}-F'$.
Thus, for every $D \subseteq V_t$, the set $D$ is compatible with ($t$, $f$) in $G_t-F^{\text{delete}}$ if and only if it is compatible with ($t'$, $f$) in $G_{t'}-F'$.
The minimum size of a set compatible with ($t$, $f$) in $G_t-F^{\text{delete}}$ is therefore $c[t',f]+\delta'(f)$.

For every $\delta'$ with $\mathrm{DP}[t',\delta'] \leq d-1$, define $\delta^{\text{delete}}(f) = +\infty$ if any of $c[t,f]$, $c[t',f]$, or $\delta'(f)$ is $+\infty$; otherwise, define $\delta^{\text{delete}}(f) = c[t',f]+\delta'(f)-c[t,f]$.
Since one additional edge is deleted, we update
\begin{align*}
  \mathrm{DP}[t,\delta^{\text{delete}}] \gets
  \min\{\mathrm{DP}[t,\delta^{\text{delete}}],\mathrm{DP}[t',\delta']+1\}.
\end{align*}

\paragraph{Forget node.}
Let $t$ be a forget node with child $t'$, where $X_t = X_{t'} \setminus \{w\}$ for some $w \in X_{t'}$.
No edge is introduced at $t$, so $E_t = E_{t'}$ and the possible edge deletion sets are the same at the two nodes.

Let $\delta'$ be a state at $t'$ realized by some $F' \subseteq E_{t'}$.
Then $F' \subseteq E_t$ and $G_t-F' = G_{t'}-F'$.
For every $D \subseteq V_t$, the set $D$ is compatible with ($t$, $f$) in $G_t-F'$ if and only if it is compatible with either ($t'$, $f_{w \to 0}$) or ($t'$, $f_{w \to 1}$) in $G_{t'}-F'$.
Indeed, $w$ must be dominated by $D$ at the parent: the case $w \notin D$ corresponds to color $0$ at the child, and the case $w \in D$ corresponds to color $1$.
Hence the minimum size of a compatible set in $G_t-F'$ is $\min\{c[t',f_{w \to 0}]+\delta'(f_{w \to 0}),c[t',f_{w \to 1}]+\delta'(f_{w \to 1})\}$.

For every $\delta'$ with $\mathrm{DP}[t',\delta'] \leq d$, define
\begin{align*}
  \delta(f) = \min\{c[t',f_{w \to 0}]+\delta'(f_{w \to 0}),
  c[t',f_{w \to 1}]+\delta'(f_{w \to 1})\}-c[t,f],
\end{align*}
with the convention that $\delta(f) = +\infty$ if either the minimum or $c[t,f]$ is $+\infty$.
We then update
\begin{align*}
  \mathrm{DP}[t,\delta] \gets \min\{\mathrm{DP}[t,\delta],\mathrm{DP}[t',\delta']\}.
\end{align*}

\paragraph{Join node.}
Let $t$ be a join node with children $t_1$ and $t_2$.
Since $E_t = E_{t_1} \cup E_{t_2}$ and $E_{t_1} \cap E_{t_2} = \emptyset$, every edge deletion set $F \subseteq E_t$ has a unique decomposition into $F_1 = F \cap E_{t_1}$ and $F_2 = F \cap E_{t_2}$.
Conversely, any $F_1 \subseteq E_{t_1}$ and $F_2 \subseteq E_{t_2}$ yield $F = F_1 \cup F_2$, with $|F| = |F_1|+|F_2|$.

Let $\delta_1$ and $\delta_2$ be realizable states at $t_1$ and $t_2$, respectively, and let $F_i \subseteq E_{t_i}$ be a minimum edge deletion set realizing $\delta_i$ for each $i \in \{1,2\}$.
Set $F = F_1 \cup F_2$.
As $F_1 \cap F_2 = \emptyset$, we have $|F| = |F_1|+|F_2|$.
If $D \subseteq V_t$ is compatible with ($t$, $f$) in $G_t-F$, then there exist colorings ($f_1$, $f_2$) consistent with $f$ such that $D_i \coloneq D \cap V_{t_i}$ is compatible with ($t_i$, $f_i$) in $G_{t_i}-F_i$ for each $i \in \{1,2\}$.
Conversely, if ($f_1$, $f_2$) are consistent with $f$ and $D_i$ is compatible with ($t_i$, $f_i$) in $G_{t_i}-F_i$ for each $i \in \{1,2\}$, then $D = D_1 \cup D_2$ is compatible with ($t$, $f$) in $G_t-F$.
The minimum size of a compatible set in $G_t-F$ is therefore
\begin{align*}
  \min_{\substack{(f_1,f_2) \\ \text{consistent with } f}}
  \{c[t_1,f_1]+\delta_1(f_1)+c[t_2,f_2]+\delta_2(f_2)-|f^{-1}(1)|\}.
\end{align*}

For every pair $(\delta_1,\delta_2)$ satisfying $\mathrm{DP}[t_1,\delta_1]+\mathrm{DP}[t_2,\delta_2] \leq d$, define
\begin{align*}
  \delta(f) = \min_{\substack{(f_1,f_2) \\ \text{consistent with } f}}
  \{c[t_1,f_1]+\delta_1(f_1)+c[t_2,f_2]+\delta_2(f_2)-|f^{-1}(1)|\}-c[t,f],
\end{align*}
with the convention that $\delta(f) = +\infty$ if either the minimum or $c[t,f]$ is $+\infty$.
This state is realized by $F = F_1 \cup F_2$, whose size is $\mathrm{DP}[t_1,\delta_1]+\mathrm{DP}[t_2,\delta_2]$.
We therefore update
\begin{align*}
  \mathrm{DP}[t,\delta] \gets
  \min\{\mathrm{DP}[t,\delta],\mathrm{DP}[t_1,\delta_1]+\mathrm{DP}[t_2,\delta_2]\}.
\end{align*}

\begin{lemma}\label{lemma:correctness}
  The transitions above correctly compute $\mathrm{DP}[t,\delta]$ for every node $t$ and state $\delta$.
\end{lemma}
\begin{proof}
  Let $\mathrm{OPT}[t,\delta]$ denote the optimum specified by the definition of the table entry.
  We prove $\mathrm{DP}[t,\delta] = \mathrm{OPT}[t,\delta]$ by induction over the tree decomposition, processing children before their parents.
  The claim holds at the leaves by initialization.
  Assume that it holds at the children of $t$.

  First, suppose that $\mathrm{DP}[t,\delta] < +\infty$.
  By the induction hypothesis and the justification of each transition, there exists an edge deletion set $F$ realizing $\delta$ with $|F| = \mathrm{DP}[t,\delta] \leq d$.
  Thus, $\mathrm{OPT}[t,\delta] \leq |F| = \mathrm{DP}[t,\delta]$.
  This inequality also holds if $\mathrm{DP}[t,\delta] = +\infty$.

  Conversely, suppose that $\mathrm{OPT}[t,\delta] < +\infty$, and let $F^*$ be a minimum edge deletion set attaining this value.
  At each node type, $F^*$ induces appropriate edge deletion sets at the children.
  At introduce vertex and forget nodes, we use $F^*$ itself at the child.
  At introduce edge nodes, we restrict $F^*$ to the child's edge set and use the transition determined by whether the introduced edge belongs to $F^*$.
  At join nodes, we split $F^*$ between the edge sets of the two children.
  By \Cref{lemma:diff}, the difference functions realized by these sets are among the states considered at the children.
  The induction hypothesis and the transition definitions imply that the corresponding transition generates $\delta$ with a value at most $|F^*|$.
  Hence $\mathrm{DP}[t,\delta] \leq |F^*| = \mathrm{OPT}[t,\delta]$.
  This inequality holds trivially if $\mathrm{OPT}[t,\delta] = +\infty$.
\end{proof}

This completes the description of the algorithm and the proof of its correctness.
We now analyze its running time.
Each bag $X_t$ has size at most $k+1$, so $|\mathcal{C}_t| = 3^{|X_t|} \leq 3^{k+1} = 3^{\mathcal{O}(k)}$.
Each state $\delta$ assigns a value in $\{0,1,\dots,d,+\infty\}$ to every coloring $f \in \mathcal{C}_t$.
Thus, the number of states at a node is at most $(d+2)^{|\mathcal{C}_t|} \leq (d+2)^{3^{k+1}} = (d+2)^{3^{\mathcal{O}(k)}}$.

At leaf, introduce vertex, introduce-edge, and forget nodes, each child state generates at most a constant number of parent states, with the leaf case handled by initialization.
Each such state can be generated in $3^{\mathcal{O}(k)}$ time by examining all colorings of the bag.
The running time at each of these nodes is therefore $(d+2)^{3^{\mathcal{O}(k)}}$.
At a join node, we examine all pairs of states from the two children.
Since each child has at most $(d+2)^{3^{\mathcal{O}(k)}}$ states, the number of pairs is at most $((d+2)^{3^{\mathcal{O}(k)}})^2 = (d+2)^{3^{\mathcal{O}(k)}}$.
For each pair of states, there are at most $4^{k+1} = 2^{\mathcal{O}(k)}$ consistent coloring triples $(f,f_1,f_2)$ to examine.
This factor is absorbed into $(d+2)^{3^{\mathcal{O}(k)}}$, so the same bound holds for the running time at a join node.
The nice tree decomposition may be assumed to have $\mathcal{O}(kn)$ nodes~\cite{DBLP:books/sp/CyganFKLMPPS15}, yielding the following result.

\begin{lemma}
  Given an $n$-vertex graph $G$ together with a tree decomposition of width at most $k$, \bondage can be solved in time $k \cdot (d+2)^{3^{\mathcal{O}(k)}} \cdot n$.
\end{lemma}

Moreover, a nice tree decomposition of width $k$ can be computed in fixed-parameter time with respect to $k$~\cite{DBLP:journals/siamcomp/Bodlaender96,DBLP:books/sp/CyganFKLMPPS15,DBLP:books/sp/Kloks94}.
We therefore obtain the following theorem.

\begin{theorem}
  The \bondage problem is fixed-parameter tractable when parameterized by $\mathrm{tw}(G)+d$, where $d$ is the solution size bound. 
\end{theorem}

The following bound relates the bondage number to treewidth.

\begin{theorem}
  For every graph $G$ without isolated vertices, $b(G) \leq 4\mathrm{tw}(G)-2$.
\end{theorem}
\begin{proof}
  Let $G = (V,E)$ be a graph of treewidth $k = \mathrm{tw}(G)$, and let $\overline{\mathrm{deg}}(G)$ denote its average degree.
  The bound $b(G) \leq 2\overline{\mathrm{deg}}(G)-1$ holds in general~\cite{DBLP:journals/dm/HartnellR99}.
  Since $G$ has treewidth $k$, we have $|E| \leq k|V|-k(k+1)/2$~\cite{DBLP:journals/siamcomp/Bodlaender96}.
  Hence $\overline{\mathrm{deg}}(G) = 2|E|/|V| \leq 2k-k(k+1)/|V| < 2k$, which implies $b(G) < 4k-1$.
  As $b(G)$ is an integer, it follows that $b(G) \leq 4k-2$.
\end{proof}

If the input bound satisfies $d \geq 4k-2$, we return \textsc{yes}; otherwise, we run the algorithm above.
In the latter case, $d$ is bounded by a function of $k$.
Combining the preceding theorems yields our main result.

\begin{theorem}
  The \bondage problem is fixed-parameter tractable when parameterized by $\mathrm{tw}(G)$. It is solvable in time $2^{2^{O(\mathrm{tw}(G))}}n$.
\end{theorem}



\subsection{Neighborhood-based parameters}\label{sec:neighbor}
\subsubsection{Neighborhood diversity}\label{sec:nd}
%\subsection{\bondage parameterized by neighborhood diversity.}

A \textit{twin class} of $G$ is a maximal set of pairwise twin vertices in $G$.
The \textit{neighborhood diversity} of $G$, denoted by $\mathrm{nd}(G)$, is the number of twin classes in $G$.
It is clear that we can compute the twin classes in $G$ in polynomial time; thus, neighborhood diversity can be computed in polynomial time.

The proof above exploits the fact that, after removing a bounded vertex set, vertices with the same neighborhood can be treated symmetrically. 
For neighborhood diversity, such a bounded partition into twin classes is available globally, which yields a simpler enumeration argument.

\begin{theorem}
    \bondage is fixed-parameter tractable parameterized by $\mathrm{nd}(G) + d$.
\end{theorem}
\begin{proof}
    Let $k = \mathrm{nd}(G)$ and let $\mathcal{U}$ denote the set of all twin classes in $G$.

    For each class $U \in \mathcal{U}$, since all vertices in $U$ are twins, there is no need to distinguish them unless they are endpoints of deleted edges.
    Let $F \subseteq E(G)$ be an edge set of size at most $d$.
    Then, at most $2d$ vertices can be incident to edges of $F$.
    Thus, if $|U| \geq 2d$, it suffices to consider only $2d$ vertices of $U$ as possible endpoints of deleted edges.
    
    Since the number of classes is $k$, and each class contains at most $2d$ vertices that we need to consider, the number of candidate vertices for endpoints of deleted edges is at most $2kd$.
    Hence, the number of candidate edges is at most $\binom{2kd}{2} = kd(2kd-1)$.
    Therefore, there are only $f(k,d)$ candidate edge sets of size at most $d$ to consider.

    We now show that, for a fixed candidate edge set $F \subseteq E(G)$, we can check whether $F$ is a solution, namely $\gamma(G-F) > \gamma(G)$.
    First, we compute $\gamma(G)$.
    This can be done in \FPT-time parameterized by $k$.
    Since $|F| \leq d$, at most $2d$ vertices can be endpoints of edges in $F$.
    We may put each of them into its own class and keep all other vertices in their original twin classes.
    Hence, we have $\mathrm{nd}(G-F) \leq k + 2d$.
    Thus, we can compute $\gamma(G-F)$ in \FPT-time parameterized by $k + d$.
    Therefore, we can check whether $\gamma(G-F) > \gamma(G)$.

    Since there are at most $f(k, d)$ candidate edge sets and each candidate can be checked in \FPT-time, we can decide whether $b(G) \leq d$ in \FPT-time parameterized by $k + d$.
    Therefore, this is a fixed-parameter algorithm parameterized by $\mathrm{nd}(G) + d$.
\end{proof}


\subsubsection{Cluster vertex deletion number}\label{sec:cd}
Let $G$ be a graph.
A set $X \subseteq V(G)$ is a cluster vertex deletion set if $G-X$ is a cluster graph, namely, each component of $G-X$ is a complete graph.
The cluster vertex deletion number of $G$, denoted by $\mathrm{cvd}(G)$, is the size of a minimum cluster vertex deletion set of $G$.

While finding a minimum cluster vertex deletion set of $G$ is \NP-hard, it is fixed-parameter tractable parameterized by $\mathrm{cvd}(G)$~\cite{DBLP:journals/mst/HuffnerKMN10}.
Thus, in designing the fixed-parameter algorithm parameterized by $\mathrm{cvd}(G)$, we may assume that a minimum cluster vertex deletion set is given.

\begin{lemma}\label{lemma:cvd}
    Let $G = (V, E)$ be a graph and let $u, v \in V$.
    If $u$ and $v$ are true twins, $\gamma(G-v) = \gamma(G)$.
\end{lemma}
\begin{proof}
    We first show that $\gamma(G-v) \geq \gamma(G)$.
    Let $D$ be a minimum dominating set of $G-v$.
    Since $u$ is dominated by $D$ in $G-v$ and $u$ and $v$ are true twins,  $D$ also dominates $v$ in $G$.
    Thus, $D$ is a dominating set of $G$, and hence $\gamma(G) \leq |D| = \gamma(G-v)$.
    
    Conversely, let $D'$ be a minimum dominating set of $G$.
    If $v \notin D'$, then $D'$ is also a dominating set of $G-v$.
    If $v \in D'$, the set $(D' \setminus \{v\}) \cup \{u\}$ is a dominating set of $G-v$, since $u$ and $v$ are true twins.
    Therefore, $\gamma(G-v) \leq |D'| = \gamma(G)$.
\end{proof}
\begin{theorem}
    \bondage is fixed-parameter tractable parameterized by $\mathrm{cvd}(G) + d$.
\end{theorem}
\begin{proof}
    Let $X$ be a cluster vertex deletion set of $G$, and let $k = |X|$.
    Let $\mathcal{C}$ denote the set of cliques of $G - X$.

    For each clique $C \in \mathcal{C}$, we partition its vertices into true twin classes according to their neighborhoods in $X$.
    Then, there are at most $2^k$ such classes in each clique.

    Let $F$ be an edge set of size at most $d$.
    For each clique $C$, if $u, v \in C$ are in the same class and neither is incident to any edge of $F$, then they are true twins in $G-F$.
    By \Cref{lemma:cvd}, we have $\gamma(G - v) = \gamma(G)$ and $\gamma((G-F) - v) = \gamma(G-F)$.
    Moreover, there is no need to distinguish between the vertices in the same class; namely, we may swap the roles of the vertices in the same class arbitrarily.
    Since $|F| \leq d$, at most $2d$ vertices can be incident to edges of $F$.
    Therefore, for each clique $C$, if there exists a class whose size is greater than $2d + 1$, we may keep only $2d + 1$ vertices in the class.
    In the following, we continue to denote the reduced graph by $G$.

    We may now assume that, for every clique $C$, each true twin class contains at most $2d+1$ vertices.
    We classify the cliques in $\mathcal{C}$ according to their types, where the type of a clique is defined by the number of vertices in each true twin class.
    Then, there are at most $(2d+2)^{2^k}$ such types.
    Note that, for each true twin class, its size is one of $\{0, 1, \dots, 2d + 1\}$.
    Thus, for each clique $C$, the number of possible patterns of at most $d$ deleted edges inside $C$ or between $C$ and $X$ is bounded by a function of $k+d$.
    We also enumerate the deleted edges with both endpoints in $X$; the number of such choices is bounded by a function of $k+d$.

    Moreover, in a deletion of at most $d$ edges, at most $d$ cliques are affected.
    Since we do not have to distinguish between cliques of the same type, it suffices to specify their types and the corresponding edge-deletion patterns. 
    Therefore, there are only $f(k,d)$ candidate edge sets to consider.

    We now show that, for a fixed candidate edge set $F \subseteq E(G)$, we can check whether $F$ is a solution, namely, whether $\gamma(G-F) > \gamma(G)$.
    First, we compute $\gamma(G)$, which can be done in \FPT-time parameterized by $k$.
    For each edge $e \in F$ whose two endpoints belong to the same clique $C \in \mathcal{C}$, we choose one of its endpoints $v_e \in C$, and let $Y$ denote the set of all such vertices.
    Since $|F| \leq d$, we have $|Y| \leq d$.
    Every deleted edge inside a clique of $G-X$ has at least one endpoint in $Y$, so $(G - F) - (X \cup Y)$ is a cluster graph.
    Hence, $X \cup Y$ is a cluster vertex deletion set of $G-F$ of size at most $k + d$, which implies that $\mathrm{cvd}(G-F) \leq k + d$.
    Therefore, we can compute $\gamma(G-F)$ in \FPT-time parameterized by $k+d$ and check whether $\gamma(G-F) > \gamma(G)$.

    Since the number of candidate edge sets is at most $f(k, d)$, and for each of them, we can check whether it is a solution, we can decide whether $b(G) \leq d$ in \FPT-time parameterized by $k + d$.
    Therefore, this is a fixed-parameter algorithm parameterized by $\mathrm{cvd}(G) + d$.
\end{proof}

==> preliminaries.tex <==
\section{Preliminaries}\label{sec:pre}

We assume that the readers are familiar with standard notions from polynomial hierarchy and parameterized complexity (see, e.g. \cite{DBLP:books/daglib/0023084,DBLP:series/txtcs/FlumG06}).
We follow the standard notations in graph theory (see, e.g. \cite{diestel2025graph}).

Two distinct vertices $u,v\in V$ are \emph{twins} if $N_G(u)\setminus\{v\}=N_G(v)\setminus\{u\}$.
They are \emph{true twins} if they are adjacent; equivalently,
$N_G[u]=N_G[v]$.

A set $D\subseteq V$ is a \emph{dominating set} of $G$ if every vertex
in $V\setminus D$ has a neighbor in $D$.
The \emph{domination number} of $G$, denoted by $\gamma(G)$, is the
minimum cardinality of a dominating set of $G$.
A set $S \subseteq V$ is a \emph{vertex cover} of $G$ if, for every edge $e \in E(G)$, we have $e \cap S \neq \emptyset$.
The \emph{vertex cover number} of $G$, denoted by $\tau(G)$, is the
minimum cardinality of a vertex cover set of $G$.

For any vertex $v \in V(G)$, let $G-v$ denote the graph obtained by deleting the vertex $v$ and edges incident to $v$.
For any edge $e \in E(G)$, let $G-e$ denote the graph obtained by deleting the edge $e$.
For any edge set $F \subseteq E(G)$, let $G - F$ denote the graph obtained by deleting the edges in $F$ from $G$, namely, $G-F = (V(G), E(G) \setminus F)$.
An edge set $F\subseteq E(G)$ is a \emph{bondage set} of $G$ if $\gamma(G-F)>\gamma(G)$.
The \emph{bondage number} of $G$, denoted by $b(G)$, is the minimum
cardinality of a bondage set of $G$.
If no such edge set exists, we set $b(G)=+\infty$.
Notice that deleting edges cannot decrease the domination number, and hence $\gamma(G-F) \geq \gamma(G)$ for every $F \subseteq E(G)$.

Throughout this paper, all graphs are finite, simple, and undirected. We may assume without loss of generality that the input graph $G$ is connected.
Indeed, if $G$ has connected components $G_1, \dots, G_r$, then $\gamma(G) = \sum_{i = 1}^{r}{\gamma(G_i)}$, and consequently $b(G) = \min_{1 \leq i \leq r}{b(G_i)}$.
Thus, the \bondage problem can be solved independently on each connected component.
We further assume that $G$ has at least two vertices.
